Localizing Open-Ontology QA Semantic Parsers in a Day Using Machine Translation

We propose Semantic Parser Localizer (SPL), a toolkit that leverages Neural Machine Translation (NMT) systems to localize a semantic parser for a new language. Our methodology is to (1) generate training data automatically in the target language by augmenting machine-translated datasets with local entities scraped from public websites, (2) add a few-shot boost of human-translated sentences and train a novel XLMR-LSTM semantic parser, and (3) test the model on natural utterances curated using human translators. We assess the effectiveness of our approach by extending the current capabilities of Schema2QA, a system for English Question Answering (QA) on the open web, to 10 new languages for the restaurants and hotels domains. Our models achieve an overall test accuracy ranging between 61% and 69% for the hotels domain and between 64% and 78% for restaurants domain, which compares favorably to 69% and 80% obtained for English parser trained on gold English data and a few examples from validation set. We show our approach outperforms the previous state-of-the-art methodology by more than 30% for hotels and 40% for restaurants with localized ontologies for the subset of languages tested. Our methodology enables any software developer to add a new language capability to a QA system for a new domain, leveraging machine translation, in less than 24 hours.

==> analysis.tex <==

\subsection{Error Analysis}
We now present an error analysis
for 5 languages (Spanish, Persian, Italian, Japanese, and Chinese) for which we have access to native speakers. 
%We produce a debugging table where each row includes the sentence in the target language, the gold program, and the predicted program, and ask each person to give us a summary of the popular problems they observe the neural model has made ranked by their number of occurrence, and for each problem provide an example. 
We perform the analysis on the validation set, as it informs the design of the pre and post processing rules as shown in Figure~\ref{fig:data_collection}.
Below we discuss common errors across the languages; the discussion on language-specific problems is included in the supplementary material.
\begin{itemize}[leftmargin=*,noitemsep]
  \item Locations are sometimes parsed incorrectly. In some examples, the review author’s name is being parsed as a location name. The copying mechanism deployed by the neural model decoder relies on the context of the sentence to identify \textit{both} the type and span of the parameter values. Thus if localization is done poorly, the model will not be able to generalize beyond a fixed ontology.
  \item Queries asking for ``X-star place" requires the parser to give results for places matching exactly X number of stars. However, due to the inherent ambiguity of the sentence the results ask can include restaurants that have an equal or higher rating.
  \item Occasionally, the parser has difficulty distinguishing between rating value and the number of reviews, especially if the original sentence makes no mention of \textit{starts} or \textit{posts} and instead uses more implicit terms like \textit{top} or \textit{best}.
  \item In some examples, the input sentence asks for information about ``this restaurant" but the program uses the user's home location instead of their current location.
\item There are human mistranslations where check-in time has been mislabeled as check-out time, or hotel's rating value has been confused as review's rating value. 
\item Translation noise in some cases can change the numbers in the sentence. For example, ``at least" / ``more than" are equivalent in DBTalk language, but it's possible that when the translation occurs the number is changed (``at least 4" $\rightarrow$ ``more than 3")
\end{itemize}


In this section, we discussed some of the common mistakes that the semantic parser makes during prediction. We believe this type of analysis should be done for any language the developer wishes to extend their system to as the final step for a quick sanity-check of their pipeline. This examination can inform the design of the system for better integration with a new language.
Further improvement can be achieved if a more careful examination is done by an expert native speaker who can identify certain sentence structures and derive language-specific templates used for data augmentation. We leave this to future work as this paper investigates automatic training data generation with no human-in-the-loop.




==> intro.tex <==
\section{Introduction}
\label{intro}

Semantic parsers are the at heart of any NLU engine where human natural language needs to be understood by machines. The applications of such systems can be broadened if more languages are supported. In this work, we present a toolkit and advocate a set of guidelines needed to build a functional parser for an arbitrary language. 
Our method enables any regular software engineer across the world to extend their semantic parsing systems to a new language without full knowledge of the formal or target language.


Semantic parsing is the task of converting natural language sentences into a meaning representation executable by machine engines. From a different perspective, this can be seen as a translation task where natural utterances are mapped into a normalized universal language, i.e.formal language. Thus it is possible that several utterances with the same \textit{semantics} in one language be mapped to the same formal representation. The same concept applies to translations of one utterance to different languages assuming the \textit{meaning} or \textit{semantics} is preserved.
Leveraging this concept, we present a toolkit that can scale a semantic parsing dataset to any language with minimal human effort.

There has been extensive work in semantic parsing area, and as a result, several datasets have been released. Some of these datasets have been extended over time to cover more languages but the cost and extensive time needed to acquire high-quality examples have decelerated further expansion.
We apply our method for two domains: \textit{Restaurants} and \textit{Hotels}on a recently proposed dataset~\cite{scheam2qa} built to support questions for virtual assistant skills of databases for several domains. Their method can synthesize language utterance paired with their DBTalk Query representation ( which is a functional subset of SQL) using schemas extracted from various websites, generic query templates, and domain-specific information. To add more linguistic variety, they use crowdsourcing platforms to collect paraphrases for a subset of the synthetic data. 


First, we present how to scale such datasets to any language using public NMT systems. This eliminates the need to train multiple MT models and having access to parallel corpora of source and target languages.
Second, we evaluate the precision and robustness of our approach by performing extensive experiments and comparing the parser accuracy with previously proposed approaches\cite{}\cite{}.
Third, our results show that you can build a functional semantic parser that can parse native utterances without observing any real sentences during training, or being tuned on a real evaluation dataset.
Fourth, we are able to achieve more competitive baseline results by minimizing the difference in the encoded representation of semantically-equivalent sentences in different languages. This will boost the accuracy when performing joint training with English, as the information from equivalent gold English example for a given translated sentence is explicitly injected during training and helps correct program prediction.
Fifth, to better understand the results, we report an error analysis of the prediction results generated by our model for 5 languages. This study gives better insight as to what improvements are needed to improve the performance. We factor errors into language-independent problems which can be fixed by improving the processing of sentences before and after translation, and language-dependent which requires some language knowledge to address.


Our contributions include the following:

1) To the best of our knowledge, this is the first semantic parsing dataset which includes more than three languages. We chose linguistically different languages to support a wide range of syntax. We hope that releasing our dataset triggers further work and research in multilingual semantic parsing.

2) We require no manual annotations for the new language dataset. This is important since access to native speakers of the target language who are familiar with the formal language is very limited.

3) We are able to preserve the entities during translation so our translated sentences automatically match in terms of entity values with the formal language in English. Whereas in previous work, \cite{boot} they train with noisy data and English data hoping the errors from MT will be mitigated by observing an English sentence mapping to the same logical form. We argue that this is an inefficient approach for two reasons: First, MT noise is injected both in the sentence structure and sentence semantics including entity values.

4) An improved neural model architecture based on BERT-LSTM and similar to mBART, which has Seq2Seq architecture using XLM-R as the encoder and LSTM decoder with attention. Although in this work, we have applied this model to multilingual semantic parsing task, its usage is broader and can be deployed for multitask and crosslingual learning for any NLP task which can be framed as question answering. We will be releasing our code and pretrained models upon publication.

==> methodology-old.tex <==
\section{Multi-Lingual Parser Generation}
\label{methodology}

Our problem is how to derive a localized semantic parser for question answering using a open ontology of localized entities from an English semantic parser and its training data, with no manual annotation and a limited amount of human translation. 

Our core idea, {\em machine translation with alignment}, is to extract the alignment information between the translated and input sentences during machine translation.  This enables us to change the English entities into localized entities.

Our SPL methodology is incorporated into the Scheme2QA toolkit to give it a multilingual capability.  Schema2QA bootstraps English semantic parsers cost-effectively for new domains. Given the schema  and a small number of manual annotations on the fields in the domain, it synthesizes as training data a large variety of complex questions using a combination of hand-curated domain-independent templates.  The sentences are annotated with their formal representation in a formal language called ThingTalk.  ThingTalk is a subset of SQL in expressiveness, but it is more tailored to natural language translation. With the addition of a small number of paraphrased sentences, it trains a neural semantic parser for the domain, which has been demonstrated to outperform commercial assistants on long-tail complex questions. More recently, automatic methods using pre-trained networks are proposed to replace manual annotation and manual paraphrases.  By integrating into Schema2QA, we can tap into the training data created for new domains using Schema2QA.  

The overall architecture of our approach is illustrated in Fig.~\ref{fig:data_collection}, which shows how the English query, ``I am looking for a sushi place near Woodland Pond'' is used to generate Italian training samples looking for ``lasagna'' in ``Via Sel Corso'', ``focacia'' in ``Mercerie'', and ``pizza'' in ``Lago di Como'', with the help of an open ontology of Italian entities.  Each of the sentences are annotated with their appropriate entities in the native language.  
\iffalse
is a toolkit that can bootstrap English semantic-parsing-based QA systems for new domains. It is based on a hand-curated set of 600 generic question templates, covering different who, what, when, where questions, which can refer to an attribute with different parts-of-speech (POS) qualifiers, such as ``a restaurant that serves Italian food'', ``an Italian restaurant'', ``a restaurant with Italian cuisine'', etc. Schema2QA requires developers to annotate each column in a table with phrases in different POS. It synthesizes complex questions with a large linguistic variety.\\
\fi
\subsection{Synthesis-Based Semantic Parsers}
\label{sec:schema2qa}
Let us first present the design of the  Schema2QA semantic parser generator~\cite{xu2020schema2qa}, which use templates to generate training data consisting of pairs of natural language utterance and its semantic representation in a formal language called ThingTalk.  ThingTalk is a subset of SQL in expressiveness, but it is more tailored to natural language translation. 

\begin{enumerate}[leftmargin=*,noitemsep]
\item
\textbf{Generic language grammar templates.} Hand-curate generic question templates to generate training samples in the target language. English has about 800 generic question templates, covering different who, what, when, where questions, which can refer to an attribute with different parts-of-speech (POS) qualifiers such as ``a restaurant that serves Italian food'', or ``an Italian restaurant''. 
\item 
\textbf{Domain annotations}. To generate training data for a specific domain, add manual annotations to indicate how each attribute of the domain can be referred to in different Parts of Speech (POS). 
\item
\textbf{Paraphrase data set}. Crowdsource workers paraphrase about 1\% of the sentences synthesized from the generic templates and the domain-specific annotations.
\item
\textbf{Augmentation with entities}.
Collect entity libraries relevant in each domain, which are then used to augment the synthesized and paraphrased sentences to create a training data set. Schema2QA proposes using existing Schema.org metadata to automatically collect these from web crawling.
\item
\textbf{Evaluation with manually-annotated crowdsourced questions.}
Collect validation and test sets of realistic questions, which are hand-annotated by an expert. The validation set is used to iteratively refine the generic templates and the annotations.
\end{enumerate}

%While repeating the above for each new language is potentially possible, it is still a lot of work that requires technical experts to know each natural language, the formal language, and the specific domain. Needless to say that access to such individuals is hard and for some applications and languages impossible.

\iffalse
% in this paper, I don't care about any of this

Schema2QA shows that it can answer questions with an open ontology by demonstrating it on questions about restaurants and hotels in the real world. 
It leverages the fact that 40\% of websites in the world have some schema.org metadata. Schema2QA automatically converts schema.org schemas into the relational database representation it uses. It scrapes websites with schema.org data for entities used in these columns.  For example, Schema2QA scrape Yelp and Hyatt to populate the entity libraries for restaurants and hotels, respectively. These entities are used to train the semantic parser, which generates queries in a language called DBTalk. Such queries can thus be applied to query dynamic content collected from the web. 
\fi

\subsection{Our Proposed Methodology}
\iffalse
Our goal is to leverage, as much as possible, the work of building English semantic parsers for all languages. English is the most widely spoken language in the world, and the majority of web content is accessible in English, which leads to wide availability of English content to start.

As we're dealing with an open-ontology application, in which the full list of entities cannot be known at 

We first observe that, if we follow steps 1-3 of the Schema2QA methodology, but use localized entities for foreign countries, 

Our overall goal is to create a question answering system that can answer questions about a domain in many different languages, within a reasonable time and cost budget. Thus, we have these
\fi

Our goal in designing the multi-lingual pipeline is (1) to leverage previous and future effort in creating English parsers as much as possible, (2) to not require annotating questions in the new language because such expertise is hard to find, and (3) to use human translators as minimally as possible.

Our proposed technique replaces the first three manual steps of the Schema2QA methodology by translating English dataset to a new language while keeping input entities intact. We need to perform steps 4 and 5, however.  In addition, we need to convert the English training data into data for the target language.  

\iffalse
\textbf{Paraphrase data set}. 
We do not use paraphrase data in training because paraphrasing in English may introduce annotation errors, and machine translation automatically provides the same benefit as human paraphrasing.  The public neural translation models tend to generate natural-looking sentences, particularly for popular language pairs.
\fi

\textbf{Step 4. Augmentation with local entities.}
A multilingual system intended to be used internationally must be able to handle queries containing local entities. We observe that schema.org is a standard worldwide, so international websites all use the same English schema properties, even though the contents are in the native language. We can scrape sites like Yelp and Wikipedia which have content in many languages. A parser trained on sentences augmented with these values is more robust to unseen entities at test time. 

\textbf{Step 5. Testing with human-translated questions.}
Instead of annotating the validation and test sets, we propose to use professional translation services to translate the validation set and the test set. This allows us to reuse annotations from English set which otherwise is impossible to collect if the developer does not know the language. Note that we do not need to translate the full validation set, but only just enough that performance will be indicative of performance on the test set.

% mehrad: eval and test are real not synthesized


\begin{figure}
\centering
%\scalebox{0.7}{\includegraphics[width=1\linewidth]{figures/data_collection.pdf}}
\hbox{\hspace{-6ex}\includegraphics[width=3.9in]{figures/multilingual-pipeline2.pdf}}
\caption{Dataset collection method used to generate translated train and part of validation splits. We obtain the test splits using human translation.}
% \vspace{-1em}
\label{fig:data_collection}
\end{figure}

\subsection{Data Set Generation}
We generate the training data for a new language by translating the English training data into the target language, with named entities replaced with local values both in the natural language utterance and the ThingTalk code. 

We start from the English dataset, obtained following the full Schema2QA's methodology (Section~\ref{sec:schema2qa}). Due to data augmentation, this dataset contains many sentences that are identical after parameter values are masked out. We remove those duplicates to reduce reduce translation time and cost.

Next, we translate the English sentences into the new language, while keeping the English parameters intact. This ensures that the translated sentence matches the annotation in terms of parameter values. 

Finally, we augment the translated sentences by replacing the English parameters in the sentence and its annotation with parameters in the target language. Figure~\ref{fig:data_collection} shows how a training sample is translated.
\TODO{Use an example to illustrate what's wrong with run-time translation. mehrad: moved example to section 3.3.2}  



\begin{table*}[htb]
\vskip 0.1in
% \fontsize{8}{10}\selectfont
\centering
\scalebox{0.7}{
\begin{tabular}{l|c|c|c|c|c}
\toprule
\multirow{3}{*}{\bf Metrics} & \multicolumn{5}{c}{\bf Dataset}  \\
\hline
\bf{}  & {\bf Overnight (Blocks)}  & {\bf Overnight (Social)} & {\bf  ATIS} & {\bf Schema2QA (Restaurants)} & {\bf Schema2QA (Hotels)} \\
\hline
\# examples & 1,305 & 2,842  & 4,433 & 508,101 & 363,101 \\
avg \# unique unigrams per example   & 6.82 & 8.65 & 7.75  & 12.16 & 12.19  \\
avg \# unique bigrams per example  & 7.44 & 8.68 & 6.99  & 11.57 & 11.62 \\
avg \# unique trigrams per example   & 6.70  & 7.90 & 6.03 & 10.59 & 10.64 \\
avg \# properties per example   & 1.94 & 1.65  & 2.56 & 2.06 & 2.03 \\
avg \# values per property  & $\leq2$ & $\leq2$ & $\leq20$  & $\geq50$ & $\geq50$   \\

\bottomrule
\end{tabular}
}
\caption{Statistical analysis of the training set for Overnight, ATIS, and schema2QA datasets. For overnight, the two domains with the lowest reported accuracies are chosen.}
\vspace{-1em}
\label{tab:train_stats}
\end{table*}

\subsubsection{Pre and Postprocessing for Translation}

% \TODO{I don't understand this why we need to do this.  Don't know what quoting means. mehrad: it is a sanity check for others who wish to use this system in their own domains}
%NOT WORTH Describing:
%To sanity check the English input dataset, we first verify that the parameter values for each entity type in the sentence and program match.  
%We requote each sample by identifying program tokens wrapped in quotation marks, sorting them by token length, and attempt to find a matching token in the sentence. Once a match is found the strings are replaced with placeholders and the matching continues for the next string on the list. 

SPL leverages public NMT models, which have been optimized to produce the correct translation for many different pairs of languages. Yet, NMT models are statistical models that can occasionally produce incorrect translations.

%Because we do not have access to their internal models, we cannot apply finetuning~\cite{qiu2020pretrained} to adapt the translators to the semantic distribution of our inputs.  
From observing typical errors of a sample of inputs, we derive a few simple preprocessing and postprocessing rules to improve the NMT results for our purpose. For example, we found that the presence or absence of punctuation marks affect translation results for Persian and Arabic more than other languages. Furthermore, for languages such as Chinese and Japanese where there is no white space delimitation between words in the sentence, the quotation marks are sometimes omitted during translation which makes entity tracking difficult. We post-process the sentence using regular expressions to split English parameters from Chinese tokens. For Marian models, we also wrap placeholders for numbers, time, date in quotation marks to ensure they are not translated. 

\iffalse
First, it is given that to achieve the best translation results the input sentence should match the data structure and semantic distribution, the NMT model has been pretrained on. Several finetuning\cite{qiu2020pretrained} approaches have been proposed to adapt neural models to new domains; however, since we use public NMT systems like Google Translate, we do not have access to their internal models and subsequent finetuning is not feasible. However, it is possible to iteratively \textit{finetune} the input sentences by doing error analysis of the translation results and discovering pre and post-processing rules until satisfying results are achieved. For example, \TODO{Describe one good example of pre or post. You can also skip this section as it is very engineering oriented. mehrad: just did above} 
\fi

\subsubsection{Parameter Substitution}
It is important that the translation model recognizes the parameters and keeps them intact.  
During translation, input tokens can be modified, transliterated, omitted, or get mapped to a new token in the target language. If the semantics of the generated utterance in the target language is changed, the original program will no longer be its annotation. For example, translation of the English sentence provided in Figure~\ref{fig:data_collection} without using our methodology is:  ``{\fontsize{8.5pt}{8.5pt}\selectfont \<\novocalize \setfarsi man beh donbaale yek forw^sgaah sw^sy dar nazdyky .hw.d jangal hastam.>}" where ``sushi" is transliterated to ``{\fontsize{8.5pt}{8.5pt}\selectfont \<\novocalize \setfarsi sw^sy>}" and ``woodland pond" is translated to ``{\fontsize{8.5pt}{8.5pt}\selectfont \<\novocalize \setfarsi .hw.d jangal>}" which is a literal translation of that location and meaningless in Farsi. \TODO{Gio: a romance or germanic language will be way more understandable to an English reader here}. Furthermore, the new entities do not match with entities provided in the target program.

A similar problem happens with back-translation: \TODO{what is "back-translation"? you have not introduced it; also, explain - it cannot be the same problem}
\TODO{Example needed} 
  
In our approach, we first identify all the entity and property values in the input sentences. We then translate each example to target language while keeping the detected values intact. We then replace each value in the sentence and program with local entities. Each sentence is replaced with 10 different entity values, to form an equal number of training examples. 
%This is especially effective for languages that change the shape of input words based on sentence context such as Arabic, Finnish, and Turkish.

\subsection{Evaluation Data}
Evaluation data is collected manually, to ensure that our test set is realistic, so high accuracy is indicative of good performance in practice. We collect the evaluation data by asking professional translators, who are native speakers of the target language, to provide the most natural written form of each sentence in their language, equivalent to how they would type their queries for a text-based virtual assistant. 

In the English sentences shown to translators, parameters are replaced with placeholders (numbers, dates) or wrapped in quotation marks (restaurant, hotel, people names, cuisine types, etc.). We ask the translators to keep the parameters intact and not translate them. The parameters in the sentences and their annotations are substituted later with local values in the target language. 


==> multilingual 6/abstract.tex <==
\begin{abstract}
%Most technologies built today only support a small set of languages. The extension of such systems to new languages is hindered due to the high cost and extensive human labor associated with creating new datasets.  

We propose Semantic Parser Localizer (SPL), a toolkit that leverages Neural Machine Translation (NMT) systems to localize a semantic parser for a new language. Our methodology is to (1) generate training data automatically in the target language by augmenting machine-translated datasets with local entities scraped from public websites, (2) add a few-shot boost of human-translated sentences and train a novel XLMR-LSTM semantic parser, and (3) test the model on natural utterances curated using human translators.

%best performance can be achieved using a few shot approach where a small proportion of the train set consists of natural human translations of utterances from the English development set. 

We assess the effectiveness of our approach by extending the current capabilities of Schema2QA, a system for English Question Answering (QA) on the open web, to 10 new languages for the restaurants and hotels domains. 
Our models achieve an overall test accuracy ranging between 61\% and 69\% for the hotels domain and between 64\% and 78\% for restaurants domain, which compares favorably to 69\% and 80\% obtained for English parser trained on gold English data and a few examples from validation set. 
We show our approach outperforms the previous state-of-the-art methodology by more than 30\% for hotels and 40\% for restaurants with localized ontologies for the subset of languages tested. 

Our methodology enables any software developer to add a new language capability to a QA system for a new domain, leveraging machine translation, in less than 24 hours. Our code is released open-source.\footnote{\footnotesize{\url{https://github.com/stanford-oval/SPL}}}

\end{abstract}


==> multilingual 6/analysis.tex <==

\subsection{Error Analysis}
We now present an error analysis
for 5 languages (Spanish, Persian, Italian, Japanese, and Chinese) for which we have access to native speakers. 
%We produce a debugging table where each row includes the sentence in the target language, the gold program, and the predicted program, and ask each person to give us a summary of the popular problems they observe the neural model has made ranked by their number of occurrence, and for each problem provide an example. 
We perform the analysis on the validation set, as it informs the design of the pre and post processing rules as shown in Figure~\ref{fig:data_collection}.
Below we discuss common errors across the languages; the discussion on language-specific problems is included in the supplementary material.
\begin{itemize}[leftmargin=*,noitemsep]
  \item Locations are sometimes parsed incorrectly. In some examples, the review author’s name is being parsed as a location name. The copying mechanism deployed by the neural model decoder relies on the context of the sentence to identify \textit{both} the type and span of the parameter values. Thus if localization is done poorly, the model will not be able to generalize beyond a fixed ontology.
  \item Queries asking for ``X-star place" requires the parser to give results for places matching exactly X number of stars. However, due to the inherent ambiguity of the sentence the results ask can include restaurants that have an equal or higher rating.
  \item Occasionally, the parser has difficulty distinguishing between rating value and the number of reviews, especially if the original sentence makes no mention of \textit{starts} or \textit{posts} and instead uses more implicit terms like \textit{top} or \textit{best}.
  \item In some examples, the input sentence asks for information about ``this restaurant" but the program uses the user's home location instead of their current location.
\item There are human mistranslations where check-in time has been mislabeled as check-out time, or hotel's rating value has been confused as review's rating value. 
\item Translation noise in some cases can change the numbers in the sentence. For example, ``at least" / ``more than" are equivalent in DBTalk language, but it's possible that when the translation occurs the number is changed (``at least 4" $\rightarrow$ ``more than 3")
\end{itemize}


In this section, we discussed some of the common mistakes that the semantic parser makes during prediction. We believe this type of analysis should be done for any language the developer wishes to extend their system to as the final step for a quick sanity-check of their pipeline. This examination can inform the design of the system for better integration with a new language.
Further improvement can be achieved if a more careful examination is done by an expert native speaker who can identify certain sentence structures and derive language-specific templates used for data augmentation. We leave this to future work as this paper investigates automatic training data generation with no human-in-the-loop.




==> multilingual 6/conclusion.tex <==
\section{Conclusion}
\label{conclusion}

% Our experimental results on challenging Schema2QA dataset show the effectiveness of our approach compared to prior work. We show that proper handling of property values coming from an open ontology, effective sharing of knowledge between semantically-equivalent sentences during training, and leveraging multilingual pre-trained encoders are key to mitigate the noise introduced during translation and shrink the accuracy gap between training on machine vs human translated data. We additionally show that including 

This paper presents SPL, a toolkit and methodology to extend and localize semantic parsers to a new language with higher accuracy, yet at a fraction of the cost compared to previous methods. SPL was incorporated into the Schema2QA toolkit to give it a multilingual capability.

SPL can be used by any developer to extend their QA system's current capabilities to a new language in less than 24 hours, leveraging professional services to translate the validation data and mature public NMT systems. We found our approach to be effective on a recently proposed QA semantic parsing dataset, which is significantly more challenging than other available multilingual datasets in terms of sentence complexity and ontology size.

Our generated datasets are automatically annotated using logical forms containing localized entities; we require no human annotations. Our model outperforms the previous state-of-the-art methodology by between 30\% and 40\% depending on the domain and the language. Our new datasets and resources are released open-source\footnote{\footnotesize{\url{https://github.com/stanford-oval/SPL}}}. Our methodology enables further investigation and creation of new benchmarks to trigger more research on this topic.

==> multilingual 6/error_analysis.tex <==
\section{Error Analysis}
\label{sec:erroranalysis}
We present an error analysis for 5 languages (Spanish, Persian, Italian, Japanese, and Chinese) for which we have access to native speakers. 

\begin{itemize}[leftmargin=*,noitemsep]
  \item Locations are sometimes parsed incorrectly. In many cases, the model struggles to distinguish an explicit mention of ``here'' from no mention at all. We suspect this is due to translation noise introducing or omitting a reference to the current location.
  \item In some examples, the review author’s name is being parsed as a location name. The copying mechanism deployed by the neural model decoder relies on the context of the sentence to identify \textit{both} the type and span of the parameter values. Thus if localization is done poorly, the model will not be able to generalize beyond a fixed ontology.
  \item Occasionally, the parser has difficulty distinguishing between rating value and the number of reviews, especially if the original sentence makes no mention of \textit{starts} or \textit{posts} and instead uses more implicit terms like \textit{top} or \textit{best}.
  \item In some examples, the input sentence asks for information about ``this restaurant" but the program uses the user's home location instead of their current location.
  \item There are human mistranslations where check-in time has been mislabeled as check-out time. Additionally, sentence ambiguity is exacerbated by the human translation step, for example, between a hotel's official star rating value and the customer's average rating value. In English, this kind of ambiguity is resolved by expert annotation flagging ambiguous sentences.
  \item Translation noise in some cases, can change the numbers in the sentence. For example, ``at least" / ``more than" are equivalent in DBTalk language, but it's possible that when the translation occurs the number is changed (``at least 4" $\rightarrow$ ``more than 3").
  \item In morphologically-rich languages (such as Italian), the entities often are not in grammatical agreement with the rest of the sentence (e.g. a feminine article precedes a masculine entity), which confuses the model on the boundaries of the entity.
\end{itemize}



==> multilingual 6/experiments.tex <==
\begin{table*}[htb]
\vskip 0.1in
% \fontsize{8}{10}\selectfont
\centering
\scalebox{0.7}{
\begin{tabular}{l|r|r|r|r|r}
\toprule
\multirow{3}{*}{\bf Metrics} & \multicolumn{5}{c}{\bf Dataset}  \\
\hline
\bf{}  & {\bf Overnight (Blocks)}  & {\bf Overnight (Social)} & {\bf  ATIS} & {\bf Schema2QA (Hotels)} & {\bf Schema2QA (Restaurants)} \\
\hline
\# attributes & 10 & 15 & 16 & 18 & 25  \\
\# examples & 1,305 & 2,842  & 4,433 & 363,101 & 508,101  \\
avg \# unique unigrams per example   & 6.82 & 8.65 & 7.75  & 12.19 & 12.16  \\
avg \# unique bigrams per example  & 7.44 & 8.68 & 6.99  & 11.62 & 11.57 \\
avg \# unique trigrams per example   & 6.70  & 7.90 & 6.03 & 10.64 & 10.59  \\
avg \# properties per example   & 1.94 & 1.65  & 2.56 & 2.03 & 2.06 \\
avg \# values per property  & $\leq2$ & $\leq2$ & $\leq20$  & $\geq100$ & $\geq100$   \\

\bottomrule
\end{tabular}
}
\vspace{-0.5em}
\caption{Statistical analysis of the training set for Overnight, ATIS, and schema2QA datasets. For overnight, the two domains with the lowest reported accuracies are chosen.}
\vspace{-1.5em}
\label{tab:train_stats}
\end{table*}
\section{Experiments}
\label{experiments}

We have implemented the full SPL methodology in the form of a tool. Developers can use the SPL tool to create a new dataset and semantic parser for their task.
We evaluate our models on the Schema2QA dataset~\cite{xu2020schema2qa}, translated to other languages using our tool. We first describe our dataset and then show our tool's accuracy, both without any human-produced training data (zero-shot) and if a small amount of human-created data in the target language is available (few-shot). In our experiments, we measure the \textit{logical form exact match} (em) accuracy, which considers the result to be correct only if the output matches the gold logical form token by token.
We additionally measure the \textit{structure match} (sm) accuracy, which measures whether the gold and predicted logical forms are identical, ignoring the parameter values. 
A large difference between exact and structure accuracy indicates that the parameters are poorly handled. 
We report results on both validation and test sets. 
We present the results for both restaurants and hotels domain in this paper.  

Our toolkit uses the Genie~\cite{geniepldi19} library for synthesis and data augmentation. Our models were implemented using the Huggingface~\cite{Wolf2019HuggingFacesTS} and GenieNLP\footnote{\footnotesize{\url{https://github.com/stanford-oval/genienlp}}} libraries.
\input{hotels}
\subsection{Dataset}
Using our approach, we have constructed a multilingual dataset based on the previously proposed Schema2QA \textit{Restaurants} and \textit{Hotels} datasets~\cite{xu2020schema2qa}. These datasets contain questions over scraped Schema.org web data, expressed using the ThingTalk query language. ThingTalk is a subset of SQL in expressiveness, but it is more tailored to natural language translation. The training sets are constructed using template-based synthesis and crowdsourced paraphrasing, while the validation and test sets are crowdsourced and manually annotated by an expert.  

We chose these two datasets as a starting point as they require understanding both complex questions and a large number of entities, many of which are not seen in training. Note that the parameters in the logical forms are \textit{aligned} with those in the input utterance: every open-ontology parameter value must appear exactly in the utterance. Table~\ref{tab:train_stats} shows the comparison of our dataset with the  Overnight~\cite{overnight} and ATIS datasets~\cite{dahl1994expanding}, which previous work has translated to other languages~\cite{bootstrap}. The Schema2QA dataset is larger, has more linguistic variety, and has significantly more possible values for each property.
The hotels domain contains 443 and 528 examples, and the restaurants domain contains 528 and 524 examples in the validation and test splits, respectively. 

We scrape Yelp, OpenTable, and TripAdvisor websites for localized ontologies on restaurants, and Hotels.com and TripAdvisor for hotels.  To ensure that some entities are unseen in validation and test, each ontology is split into two, for (1) training, and (2) validation and test.  The two splits overlap between 40\% to 50\%, depending on the domain and language. We replace the English parameters in the translated sentences with localized entities.

We have translated the Schema2QA dataset to 10 different languages, chosen to be linguistically diverse. 
To translate the training set, we use Google NMT for Farsi, Japanese, and Turkish. We use Marian for the other seven languages. Marian BLEU scores for all language pairs are available online\footnote{\footnotesize{\url{https://github.com/Helsinki-NLP/Tatoeba-Challenge/tree/master/results}}}. In our initial experiments, we found that some of the models with high reported BLEU scores, such as English to Japanese, do not produce correct translations for our dataset. Thus, we perform the following to verify each model's quality: First, we choose a subset of the English evaluation set and translate it with the corresponding Marian model. The results are then back-translated to English using Google NMT. If the meaning is not preserved for at least 90\% of the samples, we use Google NMT for that language.
%Our datasets are released open-source\footnote{\footnotesize{[Link to dataset]}} to encourage further research on multilingual semantic parsing.

We chose a subset of the validation set (75\% for hotels and 72\% for restaurants) to be professionally translated. We use this data to train our parser in a few-shot setting (Section~\ref{sec:fewshot}). The full test sets for both domains are professionally translated. 


\iffalse
We perform experiments on two of the domains used in Schema2QA.  As discussed in Section~\ref{related_work}, there are other semantic parsing multilingual datasets available, the two most popular of which are Overnight and ATIS. We did a statistical analysis on the English train sets of ATIS, two domains of Overnight, and our chosen domains from the Schema2QA dataset. The results are shown in Table~\ref{tab:train_stats}. We calculate the number of unique n-grams for each example and divide it by the number of total examples in the corpus. The same process is done to find the average number of properties. We additionally calculate the number of property values present in the ontology for each dataset. Except for the average number of properties, both schema2QA datasets are statistically more complex than Overnight and ATIS as they have more lexical variety, and their ontology is an order of magnitude bigger.
\fi

\iffalse
Aside from creating a new multilingual dataset for 10 languages which we hope to trigger further research in this area, we present extensive experimental results and provide strong baselines using different training strategies.

We designed our experiments to answer the following questions:

\begin{enumerate}
    \item Instead of generating training data for every new language and training one semantic parser for each, can we build one semantic parser for English and translate foreign language utterances to English at test time?  
    \item Does the direct translation approach presented in \cite{boot} paper achieve good results on semantic parsing datasets that are not restricted to a specific ontology and contain complex queries? Does including gold English data in train set improve the results for this experiment? 
    \item Does our proposed methodology improve the baseline performance? Do we have to evaluate our models on real utterances or can we reduce the cost and effort by using machine generated sentences for validation set as well? If the test results are similar, this suggests building a multilingual semantic parser with reasonable accuracy on native language utterance is feasible by purely relying on machine translated data for training and validating.
    \item  As evident in Table\ref{}, human translated data distribution is quite different from machine translated data. Can this difference be minimized by including human translated data in the training dataset in a few shot setting? Our hypothesis is that adding a few human utterances examples help the model generalizes better and avoids overfitting on uncommon sentence structures introduced by translation. 

\end{enumerate}
\fi

\subsection{BackTranslation: Translate at Test Time}
As our first baseline, we train an English semantic parser on the English training set; at test time, the sentence (including its entities) is translated on-the-fly from the target language to English and passed to the semantic parser. 

The experimental results are shown in Table~\ref{tab:direct_hotels}.
The results vary from a minimum of 9.7\% for Japanese to a maximum of 34.4\% for Turkish.  
Comparing the results to English, we observe about 30\% to 50\% drop in exact match accuracy. In general, the closer the language is to English in terms of semantics and syntax, the higher the BLEU score will be using NMT. The large difference between em and sm accuracies is caused by the wrong prediction of parameter values. This is expected since the entities translated to English no longer match with the annotations containing localized entities. Note that the English parser has learned to primarily copy those parameters from the sentence.
%German, Finnish, and Turkish have higher results compared to Farsi and Japanese. This can be attributed to several reasons: German and English are both West Germanic languages sharing similar alphabets and vocabularies. The other two languages have a similar grammar and sentence structure, as well as sharing some characters in their alphabet. 
%his is reasonable considering that the English semantic parser has been validated and tested on real human utterances. We observe that BackTranslation produces natural-looking sentences with variety; in fact, back translation (English $\rightarrow$ Chinese $\rightarrow$ English) has been used in previous literature for generating paraphrases~\cite{federmann-etal-2019-multilingual}.

% The difference between structure match accuracy vs. exact match accuracy is about 9\%, and it is consistent across languages, including English.
% There are two main reasons for such errors: First, the parameter value is ambiguous and can be used for two different property types. For example, a parser trained with a closed restaurant ontology can recognize the brand ``California Pizza Kitchen" as a \textit{food place}. Conversely, a parser trained on out of domain data will recognize a Kitchen \textit{food place} in California \textit{state} which serves Pizza \textit{cuisine}. Second, if the sentence is short, there is not enough context around the parameter values to inform the model of what the query is asking about. For example, the sentence ``search for kentucky fried kitchen" can be understood as any place that serves kentucky fried chicken or the famous food chain KFC.


\begin{table*}[htb]
\fontsize{8}{10}\selectfont
\centering
\begin{tabular}{l||>{\centering}p{5mm}|>{\centering}p{5mm}||c|c||c|c||c|c||c|c}

\toprule
\multirow{3}{*}{\bf Language } & \multicolumn{2}{c||}{\bf BT}  & \multicolumn{4}{c||}{\bf \experimentI} & \multicolumn{4}{c}{\bf \experimentII}  \\
\cline{2-11}
& \multicolumn{2}{c||}{\bf Test} &  \multicolumn{2}{c||}{\bf Dev} & \multicolumn{2}{c||}{\bf Test} &  \multicolumn{2}{c||}{\bf Dev} & \multicolumn{2}{c}{\bf Test} \\
\cline{2-11}
  & em & sm & em & sm & em & sm & em & sm  &em & sm \\
\hline
\multicolumn{11}{c}{\bf Hotels} \\
\hline

German & 30.4 & 50.2 & 30.2 & 55.1 & 26.9 & 50.4 & 35.7 & 56.4 & \bf 30.9 & 51.9 \\
Farsi & 19.1 & 36.0 & 23.6 & 44.2 & \bf 22.6 & 43.8 & 22.2 & 44.2 & 21.4 & 42.8 \\
Finnish & 29.2 & 46.6 & 27.8 & 53.4 & 29.1 & 52.5 & 26.9 & 51.4 & \bf 30.2 & 57.2 \\
Japanese & 15.7 & 25.2 & 20.1 & 29.4 & 19.9 & 27.3 & 21.0 & 39.3 & \bf 20.5 & 39.2 \\
Turkish & \bf 32.0 & 49.4 & 18.5 & 43.6 & 17.2 & 40.9 & 22.6 & 62.3 & 25.6 & 60.2 \\
\hline
\multicolumn{11}{c}{\bf Restaurants} \\
\hline

German & 26.9 & 51.9 & 31.3 & 62.9 & 25.8 & 60.1 & 30.3 & 61.0 & \bf 27.3 & 56.9 \\
Farsi & 14.5 & 40.8 & 20.1 & 28.2 & 15.1 & 26.2 & 22.0 & 34.1 & \bf 15.5 & 28.1 \\
Finnish & \bf 24.0 & 55.0 & 19.9 & 51.9 & 18.9 & 54.4 & 22.3 & 53.8 & 20.8 & 53.2 \\
Japanese & 9.7 & 29.8 & 19.2 & 22.1 & 18.3 & 20.6 & 22.1 & 31.6 & \bf 18.1 & 24.3 \\
Turkish & \bf 34.4 & 62.6 & 29.7 & 54.2 & 28.4 & 44.1 & 33.5 & 54.7 & 28.1 & 45.6 \\

\bottomrule
\end{tabular}
\vspace{-0.7em}
\caption{Experiment results for hotels (top rows) and restaurants (bottom rows) domain using Bootstrap and BackTranslation methods as our baseline. em and sm indicate exact and structure match accuracy respectively. We chose 5 representative languages for these experiments. Exact match accuracies for the English Test set are 64.6\% for hotels, and 68.9\% for restaurants.}
\vspace{-1.6em}
\label{tab:direct_hotels}
\end{table*}



\subsection{Bootstrap: Train with Translated Data}
As proposed by \newcite{bootstrap}, we create a new training set by using NMT to directly translate the English sentences into the target language; the logical forms containing English entities are left unmodified. This data is then used to train a semantic parser.
The results are shown in Table~\ref{tab:direct_hotels}, in the ``Bootstrap'' column. Overall, the performance of Bootstrap is comparable to the performance of BackTranslation, ranging from 15\% on Farsi restaurants to 29\% on Finnish hotels.

In a second experiment, we train a semantic parser on a dataset containing both English and translated sentences. Note that the test set is the same and contains only questions in the target language.
Training with a mixture of languages has shown improvements over single language training ~\cite{liu2020multilingual, arivazhagan2019massively}.
This experiment (shown as \experimentII in Table~\ref{tab:direct_hotels}) achieves between 16\% to 31\% accuracy outperforming \experimentVdirect for all 5 languages except for Turkish hotels and Turkish and Finnish restaurants.

Overall, these two experiments show that training with translated data can improve over translation at test time, although not by much. Furthermore, as we cannot identify the original parameters in the translated sentences, we cannot augment the training data with localized entities. This step is much needed for the neural model to generalize beyond the fixed set of values it has seen during training.
A neural semantic parser trained with Bootstrap learns to translate (or transliterate) the entity names from the foreign language representation in the sentence to the English representation in the logical form. Hence, it cannot predict the localized entities contained in the test set, which are represented in the target language.

\subsection{SPL: Semantic Parser Localizer}
There are three key components in SPL methodology: 1) Translation with alignment to ensure parameters are preserved, 2) Training with parameter-augmented machine-translated data, and 3) Boosting accuracy by adding human-translated examples to the training data simulating a few-shot setting.
Here we describe the experiments we designed to evaluate each component separately.

% \begin{adjustbox}{width=\columnwidth,center}
\begin{table*}[htb]
\fontsize{8}{10}\selectfont
% \centering
% \scalebox{0.9}{
\begin{tabular}{l|>{\centering}p{5mm}|>{\centering}p{5mm}||c|c||c|c||c|c||c|c||c|c||c|c}

\toprule
\multirow{3}{*}{\bf Language} & \multicolumn{2}{c||}{\bf BT (+Align.)} &  \multicolumn{4}{c||}{\bf  Zero-Shot SPL} & \multicolumn{4}{c||}{\bf Zero-Shot SPL (+English) }&  \multicolumn{4}{c}{\bf Few-Shot SPL}   \\
\cline{2-15}
& \multicolumn{2}{c||}{\bf Test} &  \multicolumn{2}{c||}{\bf Dev} & \multicolumn{2}{c||}{\bf Test} &  \multicolumn{2}{c||}{\bf Dev} & \multicolumn{2}{c||}{\bf Test} &  \multicolumn{2}{c||}{\bf Dev} & \multicolumn{2}{c}{\bf Test} \\
\cline{2-15}
 & em  & sm & em & sm & em & sm & em & sm & em & sm & em & sm & em & sm   \\
\hline
\multicolumn{15}{c}{\bf Hotels} \\
\hline
Arabic & 22.7 & 26.1 & 51.6 & 59.8 & 51.3 & 60.8 & 53.8 & 61.7 & 54.9 & 61.7 & 60.8 & 67.2 & \bf 61.4 & 67.0 \\
German & 51.3 & 54.2 & 70.7 & 73.6 & 61.0 & 66.1 & 70.0 & 73.3 & 65.9 & 68.0 & 77.1 & 80.2 & \bf 68.6 & 71.2 \\
Spanish & 53.4 & 55.3 & 69.0 & 72.3 & 61.6 & 68.2 & 73.1 & 76.2 & 65.3 & 70.8 & 76.3 & 80.9 & \bf 67.0 & 72.0 \\
Farsi & 51.4 & 53.1 & 63.5 & 65.0 & 58.9 & 61.0 & 70.3 & 71.7 & 58.9 & 61.8 & 77.0 & 78.9 & \bf 63.5 & 65.4 \\
Finnish & 50.8 & 54.4 & 57.9 & 59.1 & 62.5 & 66.7 & 64.2 & 65.4 & 60.3 & 65.0 & 69.3 & 70.7 & \bf 68.4 & 71.3 \\
Italian & 53.4 & 56.8 & 66.9 & 72.6 & 60.8 & 66.7 & 66.4 & 71.2 & 64.4 & 69.9 & 69.8 & 75.8 & \bf 65.7 & 71.8 \\
Japanese & 42.3 & 44.6 & 71.0 & 72.0 & 63.6 & 65.0 & 71.3 & 72.1 & 59.5 & 61.4 & 73.1 & 78.2 & \bf 67.6 & 69.3 \\
Polish & 49.8 & 52.3 & 58.7 & 62.1 & 54.9 & 59.3 & 60.0 & 63.4 & 57.6 & 60.6 & 67.7 & 71.6 & \bf 64.8 & 68.4 \\
Turkish & 55.7 & 59.5 & 69.0 & 72.5 & 60.2 & 69.1 & 73.0 & 76.9 & 64.0 & 73.3 & 77.8 & 79.6 & \bf 69.3 & 74.4 \\
Chinese & 29.2 & 32.4 & 55.9 & 60.4 & 52.8 & 58.1 & 54.6 & 59.8 & 51.1 & 56.1 & 56.7 & 67.2 & \bf 62.9 & 67.4 \\
\midrule
\multicolumn{15}{c}{\bf Restaurants} \\
\midrule
Arabic & 34.6 & 36.1 & 66.7 & 69.0 & 67.0 & 70.0 & 60.8 & 63.7 & 67.7 & 71.6 & 75.9 & 77.4 & \bf 74.6 & 79.1 \\
German & 52.3 & 55.7 & 69.4 & 71.9 & 63.0 & 65.6 & 74.4 & 76.3 & 65.3 & 68.9 & 82.6 & 84.8 & \bf 77.1 & 80.7 \\
Spanish & 58.2 & 61.3 & 68.6 & 72.1 & 67.6 & 74.0 & 70.7 & 75.0 & 67.4 & 75.2 & 82.1 & 84.7 & \bf 77.5 & 80.5 \\
Farsi & 57.8 & 62.2 & 63.0 & 64.5 & 61.8 & 62.4 & 69.0 & 70.0 & 65.5 & 66.2 & 78.0 & 78.5 & \bf 74.2 & 75.0 \\
Finnish & 53.8 & 57.1 & 63.0 & 65.4 & 58.6 & 60.3 & 63.4 & 65.1 & 59.2 & 60.5 & 72.9 & 74.9 & \bf 68.1 & 69.7 \\
Italian & 56.1 & 59.5 & 52.1 & 53.3 & 48.3 & 50.6 & 53.3 & 54.6 & 52.9 & 55.3 & 70.3 & 72.0 & \bf 69.0 & 70.5 \\
Japanese & 49.6 & 52.5 & 45.1 & 47.0 & 41.3 & 43.6 & 48.9 & 51.1 & 48.7 & 50.5 & 75.2 & 76.5 & \bf 70.5 & 72.2 \\
Polish & 49.6 & 54.0 & 50.9 & 52.7 & 51.5 & 52.7 & 55.7 & 60.8 & 56.5 & 60.7 & 65.3 & 66.1 & \bf 64.3 & 65.1 \\
Turkish & 57.8 & 61.6 & 59.6 & 61.3 & 57.8 & 60.1 & 58.7 & 60.3 & 56.1 & 58.6 & 80.3 & 81.3 & \bf 74.6 & 76.5 \\
Chinese & 42.8 & 45.5 & 56.6 & 58.8 & 46.2 & 51.1 & 64.1 & 65.6 & 57.3 & 61.6 & 69.8 & 72.1 & \bf 65.3 & 69.7 \\

\bottomrule
\end{tabular}
% }
\vspace{-0.7em}
\caption{Experiment results for hotels (top rows) and restaurants (bottom rows) domain using SPL. em and sm indicate exact and structure match accuracy respectively. Zero-shot and few-shot exact match accuracies for English test set are 64.6\% and 71.5\% for hotels, and 68.9\% and 81.6\% for restaurants.}
\vspace{-1em}
\label{tab:spl_results}
\end{table*}


\subsubsection{Test Time Translation with Alignment}
In this experiment, we run BackTranslation (BT) with alignment to understand its effect.  
We translate sentences from the foreign language to English at test time, but we use the entity aligner described in Section~\ref{sec:alignment} to copy the localized entities in the foreign language to the translated sentence before feeding it into the English semantic parser.
The results, as shown in Table~\ref{tab:spl_results}, improve by 25\% to 40\% across all languages compared to naive BT. This highlights the importance of having entities that are aligned in the sentence and the logical form, as that enables the semantic parser to copy entities from the localized ontology for correct prediction. This is evident as the exact accuracy result is close to that of structure accuracy.  

\iffalse
Specifically, the improvement in BT's accuracy when alignment is used can be attributed to the following reason
First, as parameter values are preserved during translation, they match with the entities in the program, so the model can actually predict entities from the localized ontology.

As a quick solution, one can potentially form a dictionary by finding all possible translations for each token in the ontology and use them to retrieve entity spans in the target language. However, this is not very practical simply due to having an open ontology. Furthermore, public NMT systems such as Google Translate are constantly updated and refined causing translation results to be time variant.
Second, 
\fi

\subsubsection{Training with Machine Translated Data}

In the next experiment, we apply the methodology in Section~\ref{sec:methodology} to the English dataset to create localized training data and train one semantic parser per language. We translate a portion of the validation set using human translators and combine it with the machine-translated validation data.
For all the following experiments, the model with the highest em accuracy on this set is chosen and tested on human-translated test data. 

As shown in Table~\ref{tab:spl_results}, the results obtained by this methodology outperforms all the baselines. Specifically, we achieve improvements between 33\% to 50\% over the previous state-of-the-art result, represented by the Bootstrap approach. The neural model trained on SPL data takes advantage of entity alignment in the utterance and logical form and can copy the entities directly. The exact match accuracy ranges from 53\% in Chinese to 62\% in Spanish for hotels, and from 41\% in Japanese to 68\% in Spanish for restaurants. 
Comparing to the accuracy of 65\% and 69\% for hotels and restaurants in English, respectively, we see a degradation in performance for languages that are very different from English.  Languages close to English, such as Spanish, approach the performance of English. 

% \subsection{SPL (+English): Train with Translated and English data}
%\textbf{\experimentIIIjoint}: 
\subsubsection{Adding English Training Data}
Similar to Bootstrap (+English), we also experimented with combining the original English training set with the training set generated using SPL approach. 
Except for some drops (0.3\%-4\%) in accuracy for Spanish and Turkish restaurants and Finnish and Japanese hotels, we observe about 1\% to 10\% improvement compared to when English training data is not used. 
% NOT SUBSTANTIATED (Monica): The addition of English data is mostly helpful for low-resource languages where parallel training data is limited. 
As the parser is exposed to a larger vocabulary and two potentially different grammars at once, it must learn to pay more attention to sentence semantics as opposed to individual tokens.
Additionally, the English training data contains human-paraphrased sentences, which are more natural compared to synthetic data, and add variety to the training set. 
%The process of translating a sentence by a human is similar to the process of paraphrasing it, so including paraphrase data in training is beneficial for low-resource languages.
%\TODO{PLEASE TALK ABOUT THE NUMERICAL VALUE}

%Unlike the Bootstrap experiment, the results are worse for most languages in comparison with SPL results except for 3 languages, as shown in Table \ref{tab:spl_results}. This is expected since in the target language dataset, parameters have native values and match program parameters. Thus adding more English examples only helps if the translation quality of the NMT is much lower for the target language.

%The drop in the accuracy is due to two main reasons: \TODO{do you train with only synthesized english data? what about english paraphrases?} 
%Second, the parameter values used in the foreign language are localized using our approach and are no longer in English. Thus seeing English examples with English parameters causes nothing but more confusion for the neural model's copying mechanism \TODO{why is the copy mechanism confused? it copies English from English sentence, and other language from other language sentences - this does not make sense} as we observe some English parameters present in the logical forms predicted by the model for the first 8 languages in Table~\ref{tab:spl_results}.


\subsubsection{Adding a Few Human Translation to Training Data}
\label{sec:fewshot}
In our final experiment, we add the portion of the validation set translated by humans to the training set generated using SPL. Since the validation size is much smaller than the training size (0.03\% for hotels and 0.12\% for restaurants), this is similar to a few-shot scenario where a small dataset from the test distribution is used for training. 

In Table~\ref{tab:hans} we have computed BLEU~\cite{papineni2002bleu} and TER~\cite{snover2006study} scores between machine-translated and human-translated validation data for hotels. One key takeaway is that machine-translated data has quite a different distribution than human-translated data as none of the BLUE scores are higher than 0.45. Adding a few real examples can shrink this gap and yield higher accuracy on natural sentences. 

As shown in Table~\ref{tab:spl_results}, the test results are improved significantly across all the languages for both domains.
% GC: it's a new dataset, how are you achieving a new state of the art???
% achieving new state-of-the-art results on this benchmark.
%The improvement is partly due to low overlap between train and test distributions as is evident by the low BLEU scores~\cite{papineni2002bleu} in Table~\ref{tab:bleu_hotels} and partly due to few-shot and transfer capabilities of Transformer models~\cite{brown2020language,campagna2020zeroshot,moradshahi2019hubert} attained via heavy pretraining on large corpora from different domains. 
This shows that a small addition of real training data improves the model performance significantly. The exact match accuracy varies across languages, with a low of 61.4\% on Arabic and a high of 69.3\% on Turkish for hotels, and a low of 64.3\% on Polish and a high of 77.1\% on Spanish for restaurants.  The multilingual results compare favorably with those for English.  
We show that a few-shot boost of crowdsourced evaluation data in training can also improve the English semantic parser, raising its accuracy from 65\% to 72\% for hotels, and from 69\% to 82\% for restaurants.  
The few-shot approach is particularly helpful when the training and test data are collected using different methods; this can create a new avenue for further research on multilingual tasks.

We have performed an error analysis on the results generated by the parser. At a high level, we found the biggest challenge is in recognizing entities, in particular, when entities are unseen, and when the type of the entities is ambiguous. We also found translation noise would introduce confusion for implicit concepts such as ``here''. Translation sometimes introduces or removes these concepts from the sentence. Detailed error analysis is provided in Appendix~\ref{sec:erroranalysis}.

\iffalse
To summarize, in this section, we proposed several hypothesis and tested each by evaluating our methodology and comparing the results to other baseline methods.
\experimentI method proposed in \cite{bootstrap} performs poorly on 6 diverse languages. However, the results can be improved by including the original synthesized English data in the training since that mitigates the structure and semantic noise introduced by machine translation. We additionally perform a back translation of foreign languages test data into English and test the English semantic parser on them. The results outperform both baselines again for all 6 languages. Applying SPL achieves new best results for all the languages across all different settings. We observed choosing the best model evaluated on machine translated can yield similar human test performance compared a model evaluated on human translated data for almost all languages. Adding gold English data did not help the \experimentIII results for almost all languages in contrast to the improvements obtained for \experimentII, showing the benefits of having natural training data instead of synthesized data for training. In fact, SPL translation method merges the two separate pipelines introduced in \cite{xu2020schema2qa} to generate the English dataset which is synthesizing data first, and then paraphrasing via crowdsourcing.
\fi



==> multilingual 6/hotels.tex <==


% \begin{table}[htb]
% \vskip 0.1in
% \fontsize{8}{10}\selectfont
% \centering
% \begin{tabular}{l|c|c}

% \toprule
% \bf{Language} & BLEU score (\%)  & TER score (\%)  \\
% \hline

% Arabic & 15.94 & 72.36 \\ 
% German & 37.19 & 45.49 \\ 
% Spanish & 41.99 & 39.23 \\ 
% Farsi & 20.89 & 63.51 \\ 
% Finnish & 23.66 & 52.69 \\ 
% Italian & 32.74 & 44.21 \\ 
% Japanese & 44.02 & 53.78 \\ 
% Polish & 18.52 & 62.38 \\ 
% Turkish & 26.19 & 52.83 \\ 
% Chinese & 21.73 & 76.88 \\ 

% % \specialrule{.07em}{.05em}{.05em} 

% \bottomrule
% \end{tabular}
% \caption{\TODO{this table is updated} Results for different metrics used to calculate the similarity between human translation and machine translation sentences for hotels evaluation set. Higher BLUE score and lower TER score means higher translation quality.}
% \vspace{-2.2em}
% \label{tab:bleu_hotels}
% \end{table}


%%%%%%%%%%
%%%% end hotels
%%%%%%%%%%



==> multilingual 6/intro.tex <==
\section{Introduction}
\label{intro}

Semantic parsers are the at heart of any NLU engine where human natural language needs to be understood by machines. The applications of such systems can be broadened if more languages are supported. In this work, we present a toolkit and advocate a set of guidelines needed to build a functional parser for an arbitrary language. 
Our method enables any regular software engineer across the world to extend their semantic parsing systems to a new language without full knowledge of the formal or target language.


Semantic parsing is the task of converting natural language sentences into a meaning representation executable by machine engines. From a different perspective, this can be seen as a translation task where natural utterances are mapped into a normalized universal language, i.e.formal language. Thus it is possible that several utterances with the same \textit{semantics} in one language be mapped to the same formal representation. The same concept applies to translations of one utterance to different languages assuming the \textit{meaning} or \textit{semantics} is preserved.
Leveraging this concept, we present a toolkit that can scale a semantic parsing dataset to any language with minimal human effort.

There has been extensive work in semantic parsing area, and as a result, several datasets have been released. Some of these datasets have been extended over time to cover more languages but the cost and extensive time needed to acquire high-quality examples have decelerated further expansion.
We apply our method for two domains: \textit{Restaurants} and \textit{Hotels}on a recently proposed dataset~\cite{scheam2qa} built to support questions for virtual assistant skills of databases for several domains. Their method can synthesize language utterance paired with their DBTalk Query representation ( which is a functional subset of SQL) using schemas extracted from various websites, generic query templates, and domain-specific information. To add more linguistic variety, they use crowdsourcing platforms to collect paraphrases for a subset of the synthetic data. 


First, we present how to scale such datasets to any language using public NMT systems. This eliminates the need to train multiple MT models and having access to parallel corpora of source and target languages.
Second, we evaluate the precision and robustness of our approach by performing extensive experiments and comparing the parser accuracy with previously proposed approaches\cite{}\cite{}.
Third, our results show that you can build a functional semantic parser that can parse native utterances without observing any real sentences during training, or being tuned on a real evaluation dataset.
Fourth, we are able to achieve more competitive baseline results by minimizing the difference in the encoded representation of semantically-equivalent sentences in different languages. This will boost the accuracy when performing joint training with English, as the information from equivalent gold English example for a given translated sentence is explicitly injected during training and helps correct program prediction.
Fifth, to better understand the results, we report an error analysis of the prediction results generated by our model for 5 languages. This study gives better insight as to what improvements are needed to improve the performance. We factor errors into language-independent problems which can be fixed by improving the processing of sentences before and after translation, and language-dependent which requires some language knowledge to address.


Our contributions include the following:

1) To the best of our knowledge, this is the first semantic parsing dataset which includes more than three languages. We chose linguistically different languages to support a wide range of syntax. We hope that releasing our dataset triggers further work and research in multilingual semantic parsing.

2) We require no manual annotations for the new language dataset. This is important since access to native speakers of the target language who are familiar with the formal language is very limited.

3) We are able to preserve the entities during translation so our translated sentences automatically match in terms of entity values with the formal language in English. Whereas in previous work, \cite{boot} they train with noisy data and English data hoping the errors from MT will be mitigated by observing an English sentence mapping to the same logical form. We argue that this is an inefficient approach for two reasons: First, MT noise is injected both in the sentence structure and sentence semantics including entity values.

4) An improved neural model architecture based on BERT-LSTM and similar to mBART, which has Seq2Seq architecture using XLM-R as the encoder and LSTM decoder with attention. Although in this work, we have applied this model to multilingual semantic parsing task, its usage is broader and can be deployed for multitask and crosslingual learning for any NLP task which can be framed as question answering. We will be releasing our code and pretrained models upon publication.

==> multilingual 6/intro2.tex <==
\section{Introduction}
\label{intro2}



Localization is an important step in software or website development for reaching an international audience in their native language. Localization is usually done through professional services that can translate text strings quickly into a wide variety of languages. As conversational agents are increasingly used as the new interface, how do we localize them to other languages efficiently? 

%On the other hand, when it comes to conversational agents and question answering systems, extending them to other languages is significantly more complicated.

%Many of today's software and webpages are multilingual, reaching audiences from many different countries through their native languages. Localization
%\footnote{\footnotesize{https://www.gala-global.org/industry/intro-language-industry/what-localization}}

The focus of this paper is on question answering systems that use \textit{semantic parsing}, where natural language is translated into a formal, executable representation (such as SQL). Semantic parsing typically requires a large amount of training data, which must be annotated by an expert familiar with both the natural language of interest and the formal language.
The cost of acquiring such a dataset is prohibitively expensive.  

\begin{figure}[tb]
\centering
\includegraphics[width=0.9\linewidth]{figures/multilingual-pipeline-3.pdf}
\vspace{-0.5em}
\caption{Data generation pipeline used to produce train and validation splits in a new language such as Italian. Given an input sentence in English and its annotation in the formal ThingTalk query language~\cite{xu2020schema2qa}, SPL  generates multiple examples in the target language with localized entities.}
\vspace{-1em}
\label{fig:data_collection}
\end{figure}

For English, previous work has shown it is possible to bootstrap a semantic parser without massive amount of manual annotation, by using a large, hand-curated grammar of natural language~\cite{overnight, xu2020schema2qa}. 
This approach is expensive to replicate for all languages, due to the effort and expertise required to build such a grammar. Hence, we investigate the question: \textit{Can we leverage previous work on English semantic parsers for other languages by using machine translation?} And in particular, can we do so without requiring experts in each language?

% not only is it necessary to find speakers of each natural language, but they must also be experts in the target formal language. 
\iffalse
Much progress has been made in improving the creation of semantic parsers. ~\cite{overnight} introduced the acquisition of annotated training sets with a combination of data synthesis and paraphrasing. However, this approach is costly, and the synthesized examples are relatively simple.  More recently, the Schema2QA toolkit \cite{xu2020schema2qa} shows that it is possible to create competitive parsers to answer complex questions about the structured web by manually annotating the attributes in Schema.org, a common metadata format used by many websites. They rely on a hand-curated set of about 600 generic, domain-independent templates for English. These templates have been created by experts, and it is impractical to replicate this work for all other languages, especially low-resource languages. % Potentially, it is possible to repeat this work for each new language to obtain similar results. 
\fi

% In other words, is it possible to just use professional translators we have today to localize semantic parsers?  

% \subsection{Methodology Overview}
The challenge is that a semantic parser localized to a new target language must understand questions using an ontology in the target language. For example, whereas a restaurant guide in New York may answer questions about restaurants near Times Square, the one in Italy should answer questions about restaurants near the ``Colosseo'' or ``Fontana di Trevi'' in Rome, in Italian. In addition, the parser must be able to generalize beyond a fixed set of ontology where sentences refer to entities in the target language that are unseen during training. 

%While neural machine translation (NMT) technology can handle the general structure of the question well; the parser must be able to answer questions about locale-specific real-world entities, such as hotel chains, restaurant names, and local cuisines. 
%Hence, our main challenge in localizing a semantic parser is the proper handling of entities and parameter values. 

We propose a methodology that leverages machine translation to localize an English semantic parser to a new target language, where the only labor required is manual translation of a few hundreds of annotated sentences to the target language. 
Our approach, shown in Fig.~\ref{fig:data_collection}, is to convert the English training data into training data in the target language, with all the parameter values in the questions and the logical forms substituted with local entities. Such data trains the parsers to answer questions about local entities. A small sample of the English questions from the evaluation set is translated by native speakers with no technical expertise, as a few-shot boost to the automatic training set. The test data is also manually translated to assess how our model will perform on real examples. We show that this approach can boost the accuracy on the English dataset as well from 64.6\% to 71.5\% for hotels, and from 68.9\% to 81.6\% for restaurants.

\iffalse  Our approach is to first translate the English training set into the target language using NMT systems while keeping the parameter values in the sentences intact. We then replace the parameters in translated sentences with local entities to create training and evaluation data in the target language. Additionally, 
\fi
\begin{CJK}{UTF8}{min}
\begin{table*}[tb]
\vskip 0.1in
\fontsize{7}{9}\selectfont
\centering
\begin{tabular}{c|c|c}

\toprule

\bf{Language} & \bf{Country} & {\bf Examples} \\
\hline
\multicolumn{3}{c}{\bf Hotels} \\
\hline

English & \includegraphics[width=0.03\linewidth,height=1.2em]{figures/flags/us.png} & I want a hotel near times square that has at least 1000 reviews.\\
Arabic & \includegraphics[width=0.03\linewidth,height=1.2em]{figures/flags/sa.png} & {\fontsize{6pt}{6pt}\selectfont \< ana 'aryd fndq baalqarb men msjd al.hraam y.htwy `aly 1000 t`alyq `aly al'aql.> }  \\
German & \includegraphics[width=0.03\linewidth,height=1.2em]{figures/flags/de.png}  & Ich möchte ein hotel in der nähe von marienplatz, das mindestens 1000 bewertungen hat. \\
Spanish & \includegraphics[width=0.03\linewidth,height=1.2em]{figures/flags/es.png} &  Busco un hotel cerca de puerto banús que tenga al menos 1000 comentarios.
 \\
Farsi & \includegraphics[width=0.03\linewidth,height=1.2em]{figures/flags/ir.png} & {\fontsize{6pt}{6pt}\selectfont \<\novocalize \setfarsi  htly dr nzdyky baa.g arm my_hwaahm keh .hdaaql 1000 nqd daa^sth baa^sd. > }\\
Finnish & \includegraphics[width=0.03\linewidth,height=1.2em]{figures/flags/fi.png}  & Haluan paikan helsingin tuomiokirkko läheltä hotellin, jolla on vähintään 1000 arvostelua.
\\
Italian & \includegraphics[width=0.03\linewidth,height=1.2em]{figures/flags/it.png} & Voglio un hotel nei pressi di colosseo che abbia almeno 1000 recensioni.
\\
Japanese & \includegraphics[width=0.03\linewidth,height=1.2em]{figures/flags/jp.png} &  東京スカイツリー周辺でに1000件以上のレビューがあるホテルを見せて。
 \\
Polish & \includegraphics[width=0.03\linewidth,height=1.2em]{figures/flags/pl.png}  & Potrzebuję hotelu w pobliżu zamek w malborku, który ma co najmniej 1000 ocen.
\\
Turkish & \includegraphics[width=0.03\linewidth,height=1.2em]{figures/flags/tr.png} & Kapalı carşı yakınlarında en az 1000 yoruma sahip bir otel istiyorum. \\
Chinese & \includegraphics[width=0.03\linewidth,height=1.2em]{figures/flags/cn.png} & \begin{CJK*}{UTF8}{gbsn} 我想在天安门广场附近找一家有至少1000条评论的酒店。 \end{CJK*} \\

\hline
\multicolumn{3}{c}{\bf Restaurants} \\
\hline

English & \includegraphics[width=0.03\linewidth,height=1.2em]{figures/flags/us.png} & find me a restaurant that serves burgers and is open at 14:30 . \\
Arabic & \includegraphics[width=0.03\linewidth,height=1.2em]{figures/flags/sa.png}  & {\fontsize{6pt}{6pt}\selectfont \< a`a_tr ly `aly m.t`am yqdm .t`aam al^saawrmaa w yaft.ah b.hlwl alsA`at 30:14. > } \\
German & \includegraphics[width=0.03\linewidth,height=1.2em]{figures/flags/de.png} & Finden sie bitte ein restaurant mit maultaschen essen, das um 14:30 öffnet. \\
Spanish & \includegraphics[width=0.03\linewidth,height=1.2em]{figures/flags/es.png}  &  Busque un restaurante que sirva comida paella valenciana y abra a las 14:30. \\
Farsi & \includegraphics[width=0.03\linewidth,height=1.2em]{figures/flags/ir.png} & {\fontsize{6pt}{6pt}\selectfont \<\novocalize \setfarsi rstwraany braaym peydaa kn keh ^gw^gh kebaab daa^sth baa^sd w saa`at 30:14 baaz baa^sd. > } \\
Finnish & \includegraphics[width=0.03\linewidth,height=1.2em]{figures/flags/fi.png} & Etsi minulle ravintola joka tarjoilee karjalanpiirakka ruokaa ja joka aukeaa kello 14:30 mennessä.  \\
Italian & \includegraphics[width=0.03\linewidth,height=1.2em]{figures/flags/it.png}  & Trovami un ristorante che serve cibo lasagna e apre alle 14:30. \\
Japanese & \includegraphics[width=0.03\linewidth,height=1.2em]{figures/flags/jp.png}  & 寿司フードを提供し、14:30までに開店するレストランを見つけてください。\\
Polish & \includegraphics[width=0.03\linewidth,height=1.2em]{figures/flags/pl.png} & Znajdź restaurację, w której podaje się kotlet jedzenie i którą otwierają o 14:30. \\
Turkish & \includegraphics[width=0.03\linewidth,height=1.2em]{figures/flags/tr.png} & Bana köfte yemekleri sunan ve 14:30 zamanına kadar açık olan bir restoran bul.. \\
Chinese & \includegraphics[width=0.03\linewidth,height=1.2em]{figures/flags/cn.png} & \begin{CJK*}{UTF8}{gbsn} 帮我找一家在14:30营业并供应北京烤鸭菜的餐厅。 \end{CJK*}\\


\bottomrule
\end{tabular}
\vspace{-0.5em}
\caption{Example of queries that our multilingual QA system can answer in English and 10 other languages.} %We show their transliteration in this table for simplicity of presentation.}
\vspace{-1.8em}
\label{tab:sample_data}
\end{table*}
\end{CJK}

%We also use neural machine translation to build the validation set automatically. Our methodology does not require annotating the new dataset with the formal query representation. This is important since access to native speakers of the target language who are familiar with the formal language is very limited.
%translated sentences, and test on human translated sentences.

% \subsection{Experiment Overview}
We apply our approach on the \textit{Restaurants} and \textit{Hotels} datasets introduced by \newcite{xu2020schema2qa}, which contain complex queries on data scraped from major websites. We demonstrate the efficiency of our methodology by creating neural semantic parsers for 10 languages: Arabic, German, Spanish, Persian, Finnish, Italian, Japanese, Polish, Turkish, Chinese. The models can answer complex questions about hotels and restaurants in the respective languages.
%\TODO{actually languages are not countries? which countries did you use? Saudi Arabia for Arabic? Spain for Spanish? PRC for Chinese? mehrad: yes. the main country for each language as suggested by hotels.com}
An example of a query is shown for each language and domain in Table~\ref{tab:sample_data}.
%Our approach can achieve good performance across all languages, showing its effectiveness for creating localized semantic parsers cost-efficiently. 


\iffalse
The paper is structured as follows:

First, we present how to scale such datasets to any language using public NMT systems. This eliminates the need to train multiple MT models and having access to parallel corpora of source and target languages.

Second, we evaluate the precision and robustness of our approach by performing extensive experiments and comparing the parser accuracy with previously proposed approaches\cite{}\cite{}.

Third, our results show that you can build a functional semantic parser that can parse native utterances without observing any real sentences during training or being tuned on a real validation dataset.

Fourth, to better understand the results, we report an error analysis of the prediction results generated by our model for five languages. This study gives better insight as to what improvements are needed to improve the performance. We factor errors into language-independent problems, which can be fixed by improving the processing of sentences before and after translation, and language-dependent, which requires some language knowledge to address.
\fi

% \subsection{Contributions}
Our contributions include the following:
\begin{itemize}[leftmargin=*,noitemsep]
% \setlength{\itemsep}{0pt}

\item
Semantic Parser Localizer (SPL), a new methodology to localize a semantic parser for any language for which a high-quality neural machine translation (NMT) system is available. To handle an open ontology with entities in the target language, we propose {\em machine translation with alignment}, which shows the alignment of the translated language to the input language. This enables the substitution of English entities in the translated sentences with localized entities. 
Only a couple of hundred of sentences need to be translated manually;   
no manual annotation of sentences is necessary.

%\item
%Models created by our proposed methodology can answer questions on entities in the target language required for proper localization.
\item
An improved neural semantic parsing model, based on BERT-LSTM~\cite{xu2020schema2qa} but using the XLM-R encoder. Its applicability extends beyond multilingual semantic parsing task, as it can be deployed for any NLP task that can be framed as sequence-to-sequence. Pretrained models are available for download.
\item 
Experimental results of SPL for answering questions on hotels and restaurants in 10 different languages. On average, across the 10 languages, SPL achieves a logical form accuracy of 66.7\% for hotels and 71.5\% for restaurants, which is comparable to the English parser trained with English synthetic and paraphrased data. 
% \TODO{we probably should not average across languages; mehrad: don't want to repeat what we said in the abstract} 
Our method outperforms the previous state of the art and two other strong baselines by between 30\% and 40\%, depending on the language and domain. This result confirms the importance of training with local entities.

\item 
To the best of our knowledge, ours is the first multilingual semantic parsing dataset with localized entities. Our dataset covers 10 linguistically different languages with a wide range of syntax. We hope that releasing our dataset will trigger further work in multilingual semantic parsing.

\item
SPL has been incorporated into the parser generation toolkit, Schema2QA~\cite{xu2020schema2qa}, which generates QA semantic parsers that can answer complex questions of a knowledge base automatically from its schema. With the addition of SPL, developers can easily create multilingual QA agents for new domains cost-effectively. 
\end{itemize}

\iffalse
Related work: 
We preserve the entities during translation, so our translated sentences automatically match in terms of entity values with the formal language in English. Whereas in previous work, \cite{boot}, they train with noisy data and English data, hoping the errors from MT will be mitigated by observing an English sentence mapping to the same logical form. We argue that this is an inefficient approach for two reasons: First, MT noise is injected both in the sentence structure and sentence semantics, including entity values.
\fi

\iffalse
We postulate that given the dataset in the source language, there is a more optimal approach to generate data for a new language. Semantic parsing can be framed as a translation task where natural utterances are mapped into a normalized universal language, i.e. formal language. Thus utterances with the same semantics in one language or several languages will be mapped to one formal representation. Building a functional multilingual system that can parse real utterances with native entity values from an open ontology is challenging since the parser needs to understand the input semantics and syntax across all languages to be able to generate the correct logical form with correct entity values. 
\fi


==> multilingual 6/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
%\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> multilingual 6/methodology-old.tex <==
\section{Multi-Lingual Parser Generation}
\label{methodology}

Our problem is how to derive a localized semantic parser for question answering using a open ontology of localized entities from an English semantic parser and its training data, with no manual annotation and a limited amount of human translation. 

Our core idea, {\em machine translation with alignment}, is to extract the alignment information between the translated and input sentences during machine translation.  This enables us to change the English entities into localized entities.

Our SPL methodology is incorporated into the Scheme2QA toolkit to give it a multilingual capability.  Schema2QA bootstraps English semantic parsers cost-effectively for new domains. Given the schema  and a small number of manual annotations on the fields in the domain, it synthesizes as training data a large variety of complex questions using a combination of hand-curated domain-independent templates.  The sentences are annotated with their formal representation in a formal language called ThingTalk.  ThingTalk is a subset of SQL in expressiveness, but it is more tailored to natural language translation. With the addition of a small number of paraphrased sentences, it trains a neural semantic parser for the domain, which has been demonstrated to outperform commercial assistants on long-tail complex questions. More recently, automatic methods using pre-trained networks are proposed to replace manual annotation and manual paraphrases.  By integrating into Schema2QA, we can tap into the training data created for new domains using Schema2QA.  

The overall architecture of our approach is illustrated in Fig.~\ref{fig:data_collection}, which shows how the English query, ``I am looking for a sushi place near Woodland Pond'' is used to generate Italian training samples looking for ``lasagna'' in ``Via Sel Corso'', ``focacia'' in ``Mercerie'', and ``pizza'' in ``Lago di Como'', with the help of an open ontology of Italian entities.  Each of the sentences are annotated with their appropriate entities in the native language.  
\iffalse
is a toolkit that can bootstrap English semantic-parsing-based QA systems for new domains. It is based on a hand-curated set of 600 generic question templates, covering different who, what, when, where questions, which can refer to an attribute with different parts-of-speech (POS) qualifiers, such as ``a restaurant that serves Italian food'', ``an Italian restaurant'', ``a restaurant with Italian cuisine'', etc. Schema2QA requires developers to annotate each column in a table with phrases in different POS. It synthesizes complex questions with a large linguistic variety.\\
\fi
\subsection{Synthesis-Based Semantic Parsers}
\label{sec:schema2qa}
Let us first present the design of the  Schema2QA semantic parser generator~\cite{xu2020schema2qa}, which use templates to generate training data consisting of pairs of natural language utterance and its semantic representation in a formal language called ThingTalk.  ThingTalk is a subset of SQL in expressiveness, but it is more tailored to natural language translation. 

\begin{enumerate}[leftmargin=*,noitemsep]
\item
\textbf{Generic language grammar templates.} Hand-curate generic question templates to generate training samples in the target language. English has about 800 generic question templates, covering different who, what, when, where questions, which can refer to an attribute with different parts-of-speech (POS) qualifiers such as ``a restaurant that serves Italian food'', or ``an Italian restaurant''. 
\item 
\textbf{Domain annotations}. To generate training data for a specific domain, add manual annotations to indicate how each attribute of the domain can be referred to in different Parts of Speech (POS). 
\item
\textbf{Paraphrase data set}. Crowdsource workers paraphrase about 1\% of the sentences synthesized from the generic templates and the domain-specific annotations.
\item
\textbf{Augmentation with entities}.
Collect entity libraries relevant in each domain, which are then used to augment the synthesized and paraphrased sentences to create a training data set. Schema2QA proposes using existing Schema.org metadata to automatically collect these from web crawling.
\item
\textbf{Evaluation with manually-annotated crowdsourced questions.}
Collect validation and test sets of realistic questions, which are hand-annotated by an expert. The validation set is used to iteratively refine the generic templates and the annotations.
\end{enumerate}

%While repeating the above for each new language is potentially possible, it is still a lot of work that requires technical experts to know each natural language, the formal language, and the specific domain. Needless to say that access to such individuals is hard and for some applications and languages impossible.

\iffalse
% in this paper, I don't care about any of this

Schema2QA shows that it can answer questions with an open ontology by demonstrating it on questions about restaurants and hotels in the real world. 
It leverages the fact that 40\% of websites in the world have some schema.org metadata. Schema2QA automatically converts schema.org schemas into the relational database representation it uses. It scrapes websites with schema.org data for entities used in these columns.  For example, Schema2QA scrape Yelp and Hyatt to populate the entity libraries for restaurants and hotels, respectively. These entities are used to train the semantic parser, which generates queries in a language called DBTalk. Such queries can thus be applied to query dynamic content collected from the web. 
\fi

\subsection{Our Proposed Methodology}
\iffalse
Our goal is to leverage, as much as possible, the work of building English semantic parsers for all languages. English is the most widely spoken language in the world, and the majority of web content is accessible in English, which leads to wide availability of English content to start.

As we're dealing with an open-ontology application, in which the full list of entities cannot be known at 

We first observe that, if we follow steps 1-3 of the Schema2QA methodology, but use localized entities for foreign countries, 

Our overall goal is to create a question answering system that can answer questions about a domain in many different languages, within a reasonable time and cost budget. Thus, we have these
\fi

Our goal in designing the multi-lingual pipeline is (1) to leverage previous and future effort in creating English parsers as much as possible, (2) to not require annotating questions in the new language because such expertise is hard to find, and (3) to use human translators as minimally as possible.

Our proposed technique replaces the first three manual steps of the Schema2QA methodology by translating English dataset to a new language while keeping input entities intact. We need to perform steps 4 and 5, however.  In addition, we need to convert the English training data into data for the target language.  

\iffalse
\textbf{Paraphrase data set}. 
We do not use paraphrase data in training because paraphrasing in English may introduce annotation errors, and machine translation automatically provides the same benefit as human paraphrasing.  The public neural translation models tend to generate natural-looking sentences, particularly for popular language pairs.
\fi

\textbf{Step 4. Augmentation with local entities.}
A multilingual system intended to be used internationally must be able to handle queries containing local entities. We observe that schema.org is a standard worldwide, so international websites all use the same English schema properties, even though the contents are in the native language. We can scrape sites like Yelp and Wikipedia which have content in many languages. A parser trained on sentences augmented with these values is more robust to unseen entities at test time. 

\textbf{Step 5. Testing with human-translated questions.}
Instead of annotating the validation and test sets, we propose to use professional translation services to translate the validation set and the test set. This allows us to reuse annotations from English set which otherwise is impossible to collect if the developer does not know the language. Note that we do not need to translate the full validation set, but only just enough that performance will be indicative of performance on the test set.

% mehrad: eval and test are real not synthesized


\begin{figure}
\centering
%\scalebox{0.7}{\includegraphics[width=1\linewidth]{figures/data_collection.pdf}}
\hbox{\hspace{-6ex}\includegraphics[width=3.9in]{figures/multilingual-pipeline2.pdf}}
\caption{Dataset collection method used to generate translated train and part of validation splits. We obtain the test splits using human translation.}
% \vspace{-1em}
\label{fig:data_collection}
\end{figure}

\subsection{Data Set Generation}
We generate the training data for a new language by translating the English training data into the target language, with named entities replaced with local values both in the natural language utterance and the ThingTalk code. 

We start from the English dataset, obtained following the full Schema2QA's methodology (Section~\ref{sec:schema2qa}). Due to data augmentation, this dataset contains many sentences that are identical after parameter values are masked out. We remove those duplicates to reduce reduce translation time and cost.

Next, we translate the English sentences into the new language, while keeping the English parameters intact. This ensures that the translated sentence matches the annotation in terms of parameter values. 

Finally, we augment the translated sentences by replacing the English parameters in the sentence and its annotation with parameters in the target language. Figure~\ref{fig:data_collection} shows how a training sample is translated.
\TODO{Use an example to illustrate what's wrong with run-time translation. mehrad: moved example to section 3.3.2}  



\begin{table*}[htb]
\vskip 0.1in
% \fontsize{8}{10}\selectfont
\centering
\scalebox{0.7}{
\begin{tabular}{l|c|c|c|c|c}
\toprule
\multirow{3}{*}{\bf Metrics} & \multicolumn{5}{c}{\bf Dataset}  \\
\hline
\bf{}  & {\bf Overnight (Blocks)}  & {\bf Overnight (Social)} & {\bf  ATIS} & {\bf Schema2QA (Restaurants)} & {\bf Schema2QA (Hotels)} \\
\hline
\# examples & 1,305 & 2,842  & 4,433 & 508,101 & 363,101 \\
avg \# unique unigrams per example   & 6.82 & 8.65 & 7.75  & 12.16 & 12.19  \\
avg \# unique bigrams per example  & 7.44 & 8.68 & 6.99  & 11.57 & 11.62 \\
avg \# unique trigrams per example   & 6.70  & 7.90 & 6.03 & 10.59 & 10.64 \\
avg \# properties per example   & 1.94 & 1.65  & 2.56 & 2.06 & 2.03 \\
avg \# values per property  & $\leq2$ & $\leq2$ & $\leq20$  & $\geq50$ & $\geq50$   \\

\bottomrule
\end{tabular}
}
\caption{Statistical analysis of the training set for Overnight, ATIS, and schema2QA datasets. For overnight, the two domains with the lowest reported accuracies are chosen.}
\vspace{-1em}
\label{tab:train_stats}
\end{table*}

\subsubsection{Pre and Postprocessing for Translation}

% \TODO{I don't understand this why we need to do this.  Don't know what quoting means. mehrad: it is a sanity check for others who wish to use this system in their own domains}
%NOT WORTH Describing:
%To sanity check the English input dataset, we first verify that the parameter values for each entity type in the sentence and program match.  
%We requote each sample by identifying program tokens wrapped in quotation marks, sorting them by token length, and attempt to find a matching token in the sentence. Once a match is found the strings are replaced with placeholders and the matching continues for the next string on the list. 

SPL leverages public NMT models, which have been optimized to produce the correct translation for many different pairs of languages. Yet, NMT models are statistical models that can occasionally produce incorrect translations.

%Because we do not have access to their internal models, we cannot apply finetuning~\cite{qiu2020pretrained} to adapt the translators to the semantic distribution of our inputs.  
From observing typical errors of a sample of inputs, we derive a few simple preprocessing and postprocessing rules to improve the NMT results for our purpose. For example, we found that the presence or absence of punctuation marks affect translation results for Persian and Arabic more than other languages. Furthermore, for languages such as Chinese and Japanese where there is no white space delimitation between words in the sentence, the quotation marks are sometimes omitted during translation which makes entity tracking difficult. We post-process the sentence using regular expressions to split English parameters from Chinese tokens. For Marian models, we also wrap placeholders for numbers, time, date in quotation marks to ensure they are not translated. 

\iffalse
First, it is given that to achieve the best translation results the input sentence should match the data structure and semantic distribution, the NMT model has been pretrained on. Several finetuning\cite{qiu2020pretrained} approaches have been proposed to adapt neural models to new domains; however, since we use public NMT systems like Google Translate, we do not have access to their internal models and subsequent finetuning is not feasible. However, it is possible to iteratively \textit{finetune} the input sentences by doing error analysis of the translation results and discovering pre and post-processing rules until satisfying results are achieved. For example, \TODO{Describe one good example of pre or post. You can also skip this section as it is very engineering oriented. mehrad: just did above} 
\fi

\subsubsection{Parameter Substitution}
It is important that the translation model recognizes the parameters and keeps them intact.  
During translation, input tokens can be modified, transliterated, omitted, or get mapped to a new token in the target language. If the semantics of the generated utterance in the target language is changed, the original program will no longer be its annotation. For example, translation of the English sentence provided in Figure~\ref{fig:data_collection} without using our methodology is:  ``{\fontsize{8.5pt}{8.5pt}\selectfont \<\novocalize \setfarsi man beh donbaale yek forw^sgaah sw^sy dar nazdyky .hw.d jangal hastam.>}" where ``sushi" is transliterated to ``{\fontsize{8.5pt}{8.5pt}\selectfont \<\novocalize \setfarsi sw^sy>}" and ``woodland pond" is translated to ``{\fontsize{8.5pt}{8.5pt}\selectfont \<\novocalize \setfarsi .hw.d jangal>}" which is a literal translation of that location and meaningless in Farsi. \TODO{Gio: a romance or germanic language will be way more understandable to an English reader here}. Furthermore, the new entities do not match with entities provided in the target program.

A similar problem happens with back-translation: \TODO{what is "back-translation"? you have not introduced it; also, explain - it cannot be the same problem}
\TODO{Example needed} 
  
In our approach, we first identify all the entity and property values in the input sentences. We then translate each example to target language while keeping the detected values intact. We then replace each value in the sentence and program with local entities. Each sentence is replaced with 10 different entity values, to form an equal number of training examples. 
%This is especially effective for languages that change the shape of input words based on sentence context such as Arabic, Finnish, and Turkish.

\subsection{Evaluation Data}
Evaluation data is collected manually, to ensure that our test set is realistic, so high accuracy is indicative of good performance in practice. We collect the evaluation data by asking professional translators, who are native speakers of the target language, to provide the most natural written form of each sentence in their language, equivalent to how they would type their queries for a text-based virtual assistant. 

In the English sentences shown to translators, parameters are replaced with placeholders (numbers, dates) or wrapped in quotation marks (restaurant, hotel, people names, cuisine types, etc.). We ask the translators to keep the parameters intact and not translate them. The parameters in the sentences and their annotations are substituted later with local values in the target language. 


==> multilingual 6/methodology.tex <==
\section{Multi-Lingual Parser Generation}
\label{sec:methodology}

Our goal is to localize an English semantic parser for question answering that operates on an open ontology of localized entities, with no manual annotation and a limited amount of human translation. 

\subsection{Overview}
\iffalse
Our SPL methodology is incorporated into the Schema2QA toolkit to give it a multilingual capability.  Schema2QA bootstraps English semantic parsers cost-effectively for new domains. Given the schema and a small number of manual annotations on the fields in the domain, it synthesizes as training data a large variety of complex questions using a combination of hand-curated domain-independent templates.  The sentences are annotated with their formal representation in a formal language called ThingTalk.  ThingTalk is a subset of SQL in expressiveness, but it is more tailored to natural language translation. With the addition of a few hundred paraphrased sentences, it trains a neural semantic parser for the domain, which has been demonstrated to outperform commercial assistants on long-tail complex questions about restaurants. Recently, automatic methods using pre-trained networks have been proposed to replace manual annotation and manual paraphrases~\cite{autoqa}. By integrating into Schema2QA, we can tap into the training data created for new domains using Schema2QA to create more multilingual parsers.  
\fi

Our methodology is applicable to any semantic parser for which an English dataset is available, and for which the logical form ensures that the parameters appear exactly in the input sentence. We note that many previous techniques can be used to obtain the initial English dataset in a new domain.

Our methodology consists of the following steps:
\begin{enumerate}[leftmargin=*,noitemsep]
\item Generate training data in the target language from the English training data and an ontology of localized entities, as discussed below. 

\item 
Translate evaluation and test data in English to the target language.  To ensure that our test set is realistic, so high accuracy is indicative of good performance in practice, we engage professional translators, who are native speakers of the target language.  We ask them to provide the most natural written form of each sentence in their language, equivalent to how they would type their queries for a text-based virtual assistant. 

\item Train a semantic parser to translate sentences in the target language to the logical form using the generated sentences and a few shot of the manually translated sentences. Our semantic parsing model is described in Section~\ref{sec:nn}.
\end{enumerate}

\subsection{Training Data with Localized Entities}
\label{sec:trainingdata}
The overall architecture of our approach is illustrated in Fig.~\ref{fig:data_collection}, which shows how the English query, ``I am looking for a burger place near Woodland Pond'' is used to generate Italian training samples looking for ``lasagna'' in ``Via Del Corso'', ``focaccia'' in ``Mercerie'', and ``pizza'' in ``Lago di Como'', with the help of an open ontology of Italian entities.  Each of the sentences is annotated with their appropriate entities in the native language.  
This example illustrates why we have to handle the parameters of the queries carefully. While ``burger" is translated into ``hamburger", ``Woodland Pond'', a place in New York, is translated into ``laghetto nel bosco'', which is literally a ``pond in the woods''; these entities no longer match the entities in the target logical form. 
In general, during translation, input tokens can be modified, transliterated, omitted, or get mapped to a new token in the target language. If the semantics of the generated utterance in the target language is changed, the original logical form will no longer be the correct annotation of the utterance.

After translation, we substitute the entities with localized ones, and ensure the parameters in the sentences match those in the logical form.
To do so, we add a pair of pre- and post-processing steps to the translation to improve the outcome of the translation with public NMT models, based on error analysis.
For example, we found that the presence or absence of punctuation marks affect translation results for Persian and Arabic more than other languages. Furthermore, for languages such as Chinese and Japanese, where there is no white space delimitation between words in the sentence, the quotation marks are sometimes omitted during translation, which makes entity tracking difficult. We post-process the sentence using regular expressions to split English parameters from Chinese tokens. For Marian models, we also wrap placeholders for numbers, time, date in quotation marks to ensure they are not translated either.  

\subsection{Validation and Test Data}
As discussed above, a small amount of annotated data in the target language is translated by professional translators.  We create sentences with localized entities by showing to the translators English sentences where parameters are replaced with placeholders (numbers, dates) or wrapped in quotation marks (restaurant and hotel names, cuisine types, etc.). We ask the translators to keep the parameters intact and not translate them. The parameters are substituted later with local values in the target language. 

%Because we do not have access to their internal models, we cannot apply finetuning~\cite{qiu2020pretrained} to adapt the translators to the semantic distribution of our inputs.  





==> multilingual 6/model.tex <==
\section{Model Description}
\label{model}
This section first describes our translation models, then the neural semantic parser we train with the generated data. 

\subsection{Machine Translation Models}

To translate our training data, we have experimented with both pretrained Marian models ~\cite{mariannmt} and the Google public NMT system~\cite{wu2016google} (through the Google Translate API).  Marian models have an encoder-decoder architecture similar to BART~\cite{lewis2019bart} and are available in more than 500 languages and thousands of language pairs. Although Google NMT has generally higher quality than Marian models for different languages pairs and is widely adopted by different systems, Marian is preferred for two reasons. First, Marian provides flexibility, as translation is controlled and can be tuned to generate different translations for the same sentence. Second, the cost of using Google NMT to extend our work to hundreds of languages is prohibitive. 

\begin{figure}[tb]
\centering
% \scalebox{0.7}{
\includegraphics[width=1\linewidth]{figures/heatmap.png}
% }
\vspace{-2.6em}
\caption{Cross-attention weights are shown for word-pieces in the source (X axis) and target (Y axis) language. Lighter colors correspond to higher weights. The translation is different than the one in Figure~\ref{fig:data_collection} as we are using Marian instead of GT.}
\vspace{-1.5em}
\label{fig:heatmap}
\end{figure}

\subsubsection{Marian with Alignment}
\label{sec:alignment}
To find the mapping between entities in the source and the translated language, we need to 1) detect entity spans in the output sentence, 2) align those spans with input sentence spans. We have created an alignment module, which uses the cross attention weights between the encoder and the decoder of the Marian model to align the input and output sentences. These weights show the amount of attention given to each input token when an output token is being generated. 
Figure~\ref{fig:heatmap} shows a heatmap of cross-attention weights for an English sentence and its translation in Italian. The cross-attention score for each decoder token is calculated by doing a multi-head attention~\cite{vaswani2017attention} over all encoder tokens. For the example shown in Figure~\ref{fig:heatmap}, each attention vector corresponds to one column in the heatmap.

To simplify the identification of the spans, we mark each entity in the source sentence with quotation marks, using the information in the logical form. We found empirically that the quotation marks do not change the quality of the translation. When all quotation marks are retained in the translated sentences, the spans are the contiguous tokens between quotation marks in the translated sentence.  Each quotation mark in the source is aligned with the quotation mark in the target that has the highest cross-attention score between the two. If some quotations marks are not retained, however, we find the positions in the translated sentence that share the highest cross-attention score with the quotation marks surrounding each entity, to determine its span. Once spans are detected, we override target sentence spans with source sentence spans.


\subsubsection{Alignment with Google NMT}

As we cannot access the internals of Google NMT, we localize the entities by (1)
replacing parameter values in the input sentence and logical form pairs with placeholders, (2) translating the sentences, and (3) replacing the placeholders with localized entities.  Substituting with placeholders tends to degrade translation quality because the actual parameters provide a better context for translation. 

We experimented with other methods such as 1) using a glossary-based approach where parameters are detected and masked during translation and 2) replacing parameters with values from the target language before translation.  Both show poorer translation quality.  
The former technique degrades sentence quality as masking the entity reduces context information the internal transformer model relies upon to generate target sentences. The second approach creates mixed-language sentences, requiring NMT sentences to perform code-switching. It also makes the sentences look less natural and shifts input distribution away from what public NMTs have been trained on. 
%We observed degradation in sentence quality and model performance using this approach as well.



\subsection{Semantic Parsing Model}
\label{sec:nn}
The neural semantic parser we train using our translated training data is based on the previously proposed BERT-LSTM architecture~\cite{xu2020schema2qa}, which we modify to use the XLM-R pretrained model~\cite{conneau2019unsupervised} as the encoder instead.
Our model is an encoder-decoder neural network that uses the XLM-R model as an encoder and a LSTM decoder with attention and pointer-generator~\cite{see2017get}. More details are provided in Appendix~\ref{sp_model}. As in previous work~\cite{xu2020schema2qa}, we apply rule-based preprocessing to identify times, dates, phone numbers, etc. All other tokens are lower cases and split into subwords according to the pretrained vocabulary. The same subword preprocessing is applied to entity names that are present in the output logical form.





==> multilingual 6/related_work.tex <==
\section{Related Work}
\label{related_work}

\paragraph{Multi-lingual benchmarks}
 Previous work has shown it is possible to ask non-experts to annotate large datasets for applications such as natural language inference~\cite{conneau2018xnli} and machine reading~\cite{clark2020tydi}, which has led to large cross-lingual benchmarks~\cite{hu2020xtreme}. Their approach is not suitable for semantic parsing, because it requires experts that know both the formal language and the natural language.

\paragraph{Semantic Parsing}
Semantic parsing is the task of converting natural language utterances into a formal representation of its meaning. Previous work on semantic parsing is abundant, with work dating back to the 70s~\cite{Woods1977LunarRI, 10.5555/1864519.1864543, kate2005learning, berant2013semantic}. State-of-the-art methods, based on sequence-to-sequence neural networks, require large amounts of manually annotated data~\cite{dong-lapata-2016-language, jia-liang-2016-data}. Various methods have been proposed to eliminate manually annotated data for new domains, using synthesis~\cite{overnight,DBLP:journals/corr/abs-1801-04871, geniepldi19, xu2020schema2qa, autoqa}, transfer learning~\cite{zhong2017seq2sql, decoupling2018, DBLP:journals/corr/abs-1809-08887, moradshahi2019hubert}, or a combination of both~\cite{rastogi2019towards, campagna2020zeroshot}. All these works focus mainly on the English language, and have not been applied to other languages.

\paragraph{Cross-lingual Transfer of Semantic Parsing}
\newcite{duong-etal-2017-multilingual} investigate cross-lingual transferability of knowledge from a source language to the target language by employing cross-lingual word embedding. They evaluate their approach on the English and German splits of NLmaps dataset \cite{haas-riezler-2016-corpus} and on a code-switching test set that combines English and German words in the same utterance. However, they found that joint training on English and German training data achieves competitive results compared to training multiple encoders and predicting logical form using a shared decoder. This calls for better training strategies and better use of knowledge the model can potentially learn from the dataset.

The closest work to ours is Bootstrap \cite{bootstrap}, which explores using public MT systems to generate training data for other languages. They try different training strategies and find that using a shared encoder and training on target language sentences and unmodified logical forms with English entities yields the best result. Their evaluation is done on the ATIS \cite{dahl1994expanding} and Overnight \cite{overnight} datasets, in German and Chinese. These two benchmarks have a very small number of entities. As a result, their method is unsuitable for the open ontology setting, where the semantic parser must detect entities not seen during training. 
\iffalse
We find their approach in data generation interesting but sub-optimal as they translate all tokens in the sentence including entity values. If the contextual embedding for the translated token is far away from the entity value in English, the neural model can't produce the logical form with the right entity value. They mention that errors in the MT data are mitigated when the model observes a semantically-equivalent English utterance for the same logical form. Although this observation is supported by their results, the conclusion is limited since ATIS, and Overnight datasets are extremely limited in the number of possible values they have for each entity. For example, there are only two possible people names in the Overnight dataset, namely Alice and Bob. In this work, we focus on a recently proposed QA dataset that allows users to inquire about restaurants, hotels, and people using a much more complex set of sentences.
\fi
To collect real validation and test utterances, \newcite{bootstrap} use a three-staged process to collect data from Amazon Mechanical Turkers (AMTs). They ask for three translations each per English source sentence with the hypothesis that this will collect at least one adequate translation. 
We found this approach to be less cost-effective than using professional translators. Since this process is done for the test data, it is important for the translations to be verified and have high quality. 


==> multilingual 6/results.tex <==
\subsection{Translate at Test Time}
Instead of generating training data for every new language and training one semantic parser for each, can we build only one semantic parser in the source language (English) and translate foreign language utterances to English at test time? 

We train our own semantic parser on augmented synthesized English sentences and choose the best model according to its performance on the English validation set. We then back translate the human translated test dataset and preserve the parameter values. We finally test the English semantic parser on these examples and report the results in Table~\ref{tab:back_hotels}.

The results vary between languages with a minimum of 31.18\% for Persian and a maximum of 48.32\% for Chinese. Public machine translation models like Google Translate~\cite{wu2016googles,Johnson_2017} have been trained on parallel corpora for popular pairs of languages obtained from bilingual corpora or crawled and aligned from wikipeida. Persian is a mid-resource language without a lot of existing bilingual corpora in contrast to Chinese. We posit there should be a direct correlation between the results present in Table~\ref{tab:back_hotels} and the amount of pretraining Google Translate neural model has had for that language.

Comparing the results to English we observe about a 20\% drop in exact match accuracy. Since the English semantic parser has been validated and tested on real human utterances is it unreasonable to expect high results on translated human utterances. Additionally, BackTranslation introduces more natural-looking sentences with more variation. In fact back translation (English $\rightarrow$ Chinese $\rightarrow$ English) has been used in previous literature for generating paraphrases~\cite{federmann-etal-2019-multilingual}.

Structure match accuracy (which compares predicted and gold program after removing parameter) tokens shows an improvement for about 9\% over Exact match accuracy (where parameters are considered when calculating the score). The difference is more or less the same across different languages and the same as English, suggesting that if the parser is having difficulty detecting the right parameter in the real English utterance, changing the context around that value would not help much. This can be caused in two cases:

\begin{enumerate}
    \item The parameter value is ambiguous and can be used for two different property types. For example, the word ``California Pizza Kitchen" to a parser that has been trained with restaurant domain data is a \textit{food place}. Whereas for a parser trained on out of domain data is a Kitchen \textit{place} in California \textit{state} which serves Pizza \textit{cuisine}.
    \item The context around the parameter value is short and does not inform the model of what the query is asking about. For example, the sentence ``search for italian", can be understood by the model asking for a place that serves italian cuisine or a food place named italian.
\end{enumerate}

  


% \TODO{What do the results say?  Summarize the range of results.  Why are Japanese and Chinese so bad? What are the common problems that make the accuracy drop about 20\% Is it a bug or is it real?   The answer is we lose on average 25\% for all languages except for Japanese and Chinese that are hopeless.
% What is the difference between em and sm. What is the drop between em and sm? Characterize and discuss. Does this difference remain the same across the different languages and different expt setups? 
% }

\subsection{Train with Machine Translated Sentences}
Does the direct translation approach presented in \cite{bootstrap} achieve good results on semantic parsing datasets that are not restricted to a specific ontology and contain complex queries? Does including gold English data in train set improve the results for this experiment? 

% \TODO{I don't know why it is called DIRECT. mehrad: there is no processing here: Sentence in, translation out. Direct with no additional branches in the methodology graph.}

We perform the two following experiments on only a subset of the languages. The subset is chosen to maximize structure diversity as each language is representative of a different linguistic phenomena.

\textbf{\experimentI}: We create the train set for each language by directly translating the gold English training split using NMT, without preserving parameter values, or augmenting them in the target language. We then evaluate and test on human translated data.
Results are shown in Table \ref{tab:direct_hotels} ranging between 14\% to 25\%   which is significantly worse than \experimentV results for all 6 languages. The reason for this drop is twofold:
1) As parameter values are not preserved during translation, they can either get translated, transliterated, or mapped to certain token(s) depending on the context. Furthermore, the mapping is not done deterministically since public APIs we use for translation are constantly updated and refined via more translation data and human corrections. One can potentially form a database by finding all possible translations for every token in the ontology and match values by looking them up in this table. Aside from being costly, this is not a feasible approach simply due to having an open ontology for real systems deployed across the globe.
2) Since we are not able to identify the original parameters in the translated sentence using this approach, augmentation with real parameters from the native library is not possible. This step is much needed for the neural model to be able to generalize beyond the fixed set of values it has seen during training.


% \TODO{Discuss the range of direct.  A smaller range, with Japanese becoming one of the strongest languages.  Why? We probably need to summarize each result with the range, and perhaps an average.  
% You can use Persian to explain the difference between Direct and BackTranslation.  Describe the range of difference with Backtranslation.  
% To get a sense of how to compare across techniques.  
%  What happens to Japanese?}


\textbf{\experimentII}: We follow the same procedure as the previous approach, but include gold English examples in the training set too.
The test results show about 5\% and 10\% improvement on German and Turkish, both of which are left to right languages sharing similar alphabet as English. This shows the power of our neural in incorporating structure knowledge for cross-lingual training. The results improve by small amounts for Arabic while it drops for Persian and Japanese. Japanese writing system uses a combination of logographic kanji and syllabic kana, while Persian/ Arabic uses Perso-Arabic alphabet adopted from Cyrillic alphabet both of which have not lexical overlap with English characters. 
    
% \TODO{Why does Gold improves 2 languages. }

\subsection{Semantic Parser Localizer (SPL)}
Can our proposed methodology improve baseline performance? Do we have to evaluate our models on real utterances or can the machine translated sentences serve as a good substitute? If the test results are close, this suggests building a multilingual semantic parser with reasonable accuracy on native language utterance is feasible by purely relying on machine translated data for training and validation.

We evaluate SPL in four different settings, the details of which are as follows:

\textbf{\experimentIII}: We generate the training set for each language by applying our methodology on the training English dataset. We then train one semantic parser for each language by evaluating and testing on human translated validation and test dataset.\\

\textbf{\experimentIV}: The training set is the same as the previous approach. However, we evaluate our models on the Machine Translated (MT) development set. For some languages such as Arabic, Spanish, and Japanese this method outperforms \experimentIII results where the difference is bolder for Arabic. For other languages, the test results are still competitive with drops ranging from 3\% for German to 8\% for Polish and Chinese. The results highly depend on the quality of machine translated data since the model is now being trained and evaluated on the data from the same distribution but tested on human translated utterances. However, the relatively small gap between \experimentIII and \experimentIV results suggest that it is possible to build a functional semantic parser for other languages by entirely relying on machine generated data for training and evaluation. 

Furthermore, we perform a quantitative analysis by calculating the similarity between machine and human translated sentences in the validation set to discover if there are any correlations between these scores and experimental results for \experimentIII and \experimentIV.
The computed metrics are:
1) Bilingual Evaluation Understudy (BLEU) score which is a popular n-gram based approach showing a high correlation with human judgments of sentence quality. 2) Translation Error Rate (TER) score which measures the number of edits a translator needs to perform on machine translated text so it exactly matches human translated sentence.
We calculate both of these scores per sentence and then average across the corpus. The results are presented in Table \ref{tab:bleu_hotels}. We use percentages instead of absolute numbers in the Table. Spanish and Japanese have relatively high BLEU scores which correlate with the small gap in the accuracy numbers for \experimentIII and \experimentIV experiments.
The correlation is, however, less obvious for Arabic. Persian has the lowest BLEU score among all languages which corresponds with the 6\% in accuracy compared to tuning on human utterances.\\
Overall, the results obtained by applying our methodology outperforms all the previous baselines (\experimentI, \experimentII, \experimentV) for all languages we did experiment on. Specifically, we achieve improvements between 17\% to 33\% over the \experimentV results. This attests to the strength of having a large, automatically synthesized training set with localized parameters.

\textbf{\experimentIIIjoint}: We perform a similar experiment as \experimentI, by including augmented English dataset in our training data, and training jointly on both languages. The results are worse for most languages in comparison with \textbf{\experimentIV} results except for 3 languages. This is expected since, in the target language dataset, parameters have native values and match program parameters. Thus adding more English examples only helps if the translation quality of the NMT is much lower for the target language. Table \ref{tab:spl_hotels} shows that test accuracy drops for 8 languages compared to \experimentIII except for Turkish, Chinese, and Japanese; whereas including gold English in \experimentII was helping most of the languages. This shows that our translated datasets are robust and informative enough that mixing them with data from another language would not improve the performance by a lot and in some cases can even hurt the results. The drop in the accuracy is caused due to two main reasons:\\
1) Our training dataset for each foreign language is generated by machine translation. The outputs are more natural-looking than synthesized English data even though they might not have correct grammar structure. Mixing distributions in train set is not a good approach especially since we validate and test on natural utterances.\\
2) The parameter values used in the foreign language are localized using our approach and are no longer in English. Thus seeing English examples with English parameters causes nothing but more confusion for the neural model's copying mechanism as we observe some English parameters present in the logical forms predicted by the model for the top 8 languages in Table~\ref{tab:spl_hotels}.

% since gold English sentences can be used to infer the correct program parameters and mitigates the structure and semantic noise introduced by direct translation. 
% \TODO{Discuss the numbers}

\subsection{Training with Human Translated Sentences}
As evident in Table~\ref{tab:bleu_hotels}, human translated data distribution is quite different from machine translated data. Can this difference be minimized by including human translated data in the training dataset in a few shot setting? Our hypothesis is that adding a few human utterances examples help the model generalizes better and avoids overfitting on uncommon sentence structures introduced by translation. 
 
\textbf{\experimentVII} In our final experiment, we concatenate the validation set obtained by humans to the training set generated using SPI. Since the validation size is much smaller than the training size (0.03\% for hotels and 0.12\% for restaurants) this is similar to a few-shot scenario where a small set of examples from eval/ test distribution are used for training.
We also create a new validation set by concatenating the machine and human translated examples from the validation set. This is to avoid overfitting on human data as we have included that in the training set. We then train the semantic parser on the joint train set and evaluate on the mixed development set. We experimented by evaluating only on machine translated validation data too but the results were lower. 

As shown in Table~\ref{tab:spl_hotels}, the test results are improved significantly across 9 languages for hotels domain achieving new state-of-the-art results on this benchmark. The improvement is partly due to low overlap between the train and test distributions as is evident by the low BLEU scores in Table\ref{tab:bleu_hotels} and partly due to few-shot and transfer capabilities of transformer models~\cite{brown2020language,campagna2020zeroshot,moradshahi2019hubert} attained via heavy pretraining on large corpora from different domains. 

We believe the parsing accuracy can be further boosted by adding more natural sentences collected via native speakers. We posit there is a threshold after which the cost of acquiring new examples outweighs the accuracy gain, but this investigation is out of the scope of this paper and will be explored in future work.

To summarize, in this section, we proposed several hypotheses and tested each by evaluating our methodology and comparing the results to other baseline methods.
\experimentI method proposed in \cite{bootstrap} performs poorly on 6 diverse languages. However, the results can be improved by including the original synthesized English data in the training since that mitigates the structure and semantic noise introduced by machine translation. We additionally perform a back translation of foreign languages test data into English and test the English semantic parser on them. The results outperform both baselines again for all 6 languages. Applying SPL achieves new best results for all the languages across all different settings. We observed choosing the best model evaluated on machine translated can yield similar human test performance compared to a model evaluated on human translated data for almost all languages. Adding gold English data did not help the \experimentIII results for almost all languages in contrast to the improvements obtained for \experimentII, speaking to the benefits of having training data instead of synthesized data for training. In fact, SPL translation method merges the two separate pipelines introduced in \cite{xu2020schema2qa} to generate the English dataset which is data synthesis and human paraphrasing. 
    
% \TODO{Discuss the numbers like the above.  What are the conclusions?}
 
%%%%%%%%%%
%%%% begin hotels
%%%%%%%%%%


==> results.tex <==
\subsection{Translate at Test Time}
Instead of generating training data for every new language and training one semantic parser for each, can we build only one semantic parser in the source language (English) and translate foreign language utterances to English at test time? 

We train our own semantic parser on augmented synthesized English sentences and choose the best model according to its performance on the English validation set. We then back translate the human translated test dataset and preserve the parameter values. We finally test the English semantic parser on these examples and report the results in Table~\ref{tab:back_hotels}.

The results vary between languages with a minimum of 31.18\% for Persian and a maximum of 48.32\% for Chinese. Public machine translation models like Google Translate~\cite{wu2016googles,Johnson_2017} have been trained on parallel corpora for popular pairs of languages obtained from bilingual corpora or crawled and aligned from wikipeida. Persian is a mid-resource language without a lot of existing bilingual corpora in contrast to Chinese. We posit there should be a direct correlation between the results present in Table~\ref{tab:back_hotels} and the amount of pretraining Google Translate neural model has had for that language.

Comparing the results to English we observe about a 20\% drop in exact match accuracy. Since the English semantic parser has been validated and tested on real human utterances is it unreasonable to expect high results on translated human utterances. Additionally, BackTranslation introduces more natural-looking sentences with more variation. In fact back translation (English $\rightarrow$ Chinese $\rightarrow$ English) has been used in previous literature for generating paraphrases~\cite{federmann-etal-2019-multilingual}.

Structure match accuracy (which compares predicted and gold program after removing parameter) tokens shows an improvement for about 9\% over Exact match accuracy (where parameters are considered when calculating the score). The difference is more or less the same across different languages and the same as English, suggesting that if the parser is having difficulty detecting the right parameter in the real English utterance, changing the context around that value would not help much. This can be caused in two cases:

\begin{enumerate}
    \item The parameter value is ambiguous and can be used for two different property types. For example, the word ``California Pizza Kitchen" to a parser that has been trained with restaurant domain data is a \textit{food place}. Whereas for a parser trained on out of domain data is a Kitchen \textit{place} in California \textit{state} which serves Pizza \textit{cuisine}.
    \item The context around the parameter value is short and does not inform the model of what the query is asking about. For example, the sentence ``search for italian", can be understood by the model asking for a place that serves italian cuisine or a food place named italian.
\end{enumerate}

  


% \TODO{What do the results say?  Summarize the range of results.  Why are Japanese and Chinese so bad? What are the common problems that make the accuracy drop about 20\% Is it a bug or is it real?   The answer is we lose on average 25\% for all languages except for Japanese and Chinese that are hopeless.
% What is the difference between em and sm. What is the drop between em and sm? Characterize and discuss. Does this difference remain the same across the different languages and different expt setups? 
% }

\subsection{Train with Machine Translated Sentences}
Does the direct translation approach presented in \cite{bootstrap} achieve good results on semantic parsing datasets that are not restricted to a specific ontology and contain complex queries? Does including gold English data in train set improve the results for this experiment? 

% \TODO{I don't know why it is called DIRECT. mehrad: there is no processing here: Sentence in, translation out. Direct with no additional branches in the methodology graph.}

We perform the two following experiments on only a subset of the languages. The subset is chosen to maximize structure diversity as each language is representative of a different linguistic phenomena.

\textbf{\experimentI}: We create the train set for each language by directly translating the gold English training split using NMT, without preserving parameter values, or augmenting them in the target language. We then evaluate and test on human translated data.
Results are shown in Table \ref{tab:direct_hotels} ranging between 14\% to 25\%   which is significantly worse than \experimentV results for all 6 languages. The reason for this drop is twofold:
1) As parameter values are not preserved during translation, they can either get translated, transliterated, or mapped to certain token(s) depending on the context. Furthermore, the mapping is not done deterministically since public APIs we use for translation are constantly updated and refined via more translation data and human corrections. One can potentially form a database by finding all possible translations for every token in the ontology and match values by looking them up in this table. Aside from being costly, this is not a feasible approach simply due to having an open ontology for real systems deployed across the globe.
2) Since we are not able to identify the original parameters in the translated sentence using this approach, augmentation with real parameters from the native library is not possible. This step is much needed for the neural model to be able to generalize beyond the fixed set of values it has seen during training.


% \TODO{Discuss the range of direct.  A smaller range, with Japanese becoming one of the strongest languages.  Why? We probably need to summarize each result with the range, and perhaps an average.  
% You can use Persian to explain the difference between Direct and BackTranslation.  Describe the range of difference with Backtranslation.  
% To get a sense of how to compare across techniques.  
%  What happens to Japanese?}


\textbf{\experimentII}: We follow the same procedure as the previous approach, but include gold English examples in the training set too.
The test results show about 5\% and 10\% improvement on German and Turkish, both of which are left to right languages sharing similar alphabet as English. This shows the power of our neural in incorporating structure knowledge for cross-lingual training. The results improve by small amounts for Arabic while it drops for Persian and Japanese. Japanese writing system uses a combination of logographic kanji and syllabic kana, while Persian/ Arabic uses Perso-Arabic alphabet adopted from Cyrillic alphabet both of which have not lexical overlap with English characters. 
    
% \TODO{Why does Gold improves 2 languages. }

\subsection{Semantic Parser Localizer (SPL)}
Can our proposed methodology improve baseline performance? Do we have to evaluate our models on real utterances or can the machine translated sentences serve as a good substitute? If the test results are close, this suggests building a multilingual semantic parser with reasonable accuracy on native language utterance is feasible by purely relying on machine translated data for training and validation.

We evaluate SPL in four different settings, the details of which are as follows:

\textbf{\experimentIII}: We generate the training set for each language by applying our methodology on the training English dataset. We then train one semantic parser for each language by evaluating and testing on human translated validation and test dataset.\\

\textbf{\experimentIV}: The training set is the same as the previous approach. However, we evaluate our models on the Machine Translated (MT) development set. For some languages such as Arabic, Spanish, and Japanese this method outperforms \experimentIII results where the difference is bolder for Arabic. For other languages, the test results are still competitive with drops ranging from 3\% for German to 8\% for Polish and Chinese. The results highly depend on the quality of machine translated data since the model is now being trained and evaluated on the data from the same distribution but tested on human translated utterances. However, the relatively small gap between \experimentIII and \experimentIV results suggest that it is possible to build a functional semantic parser for other languages by entirely relying on machine generated data for training and evaluation. 

Furthermore, we perform a quantitative analysis by calculating the similarity between machine and human translated sentences in the validation set to discover if there are any correlations between these scores and experimental results for \experimentIII and \experimentIV.
The computed metrics are:
1) Bilingual Evaluation Understudy (BLEU) score which is a popular n-gram based approach showing a high correlation with human judgments of sentence quality. 2) Translation Error Rate (TER) score which measures the number of edits a translator needs to perform on machine translated text so it exactly matches human translated sentence.
We calculate both of these scores per sentence and then average across the corpus. The results are presented in Table \ref{tab:bleu_hotels}. We use percentages instead of absolute numbers in the Table. Spanish and Japanese have relatively high BLEU scores which correlate with the small gap in the accuracy numbers for \experimentIII and \experimentIV experiments.
The correlation is, however, less obvious for Arabic. Persian has the lowest BLEU score among all languages which corresponds with the 6\% in accuracy compared to tuning on human utterances.\\
Overall, the results obtained by applying our methodology outperforms all the previous baselines (\experimentI, \experimentII, \experimentV) for all languages we did experiment on. Specifically, we achieve improvements between 17\% to 33\% over the \experimentV results. This attests to the strength of having a large, automatically synthesized training set with localized parameters.

\textbf{\experimentIIIjoint}: We perform a similar experiment as \experimentI, by including augmented English dataset in our training data, and training jointly on both languages. The results are worse for most languages in comparison with \textbf{\experimentIV} results except for 3 languages. This is expected since, in the target language dataset, parameters have native values and match program parameters. Thus adding more English examples only helps if the translation quality of the NMT is much lower for the target language. Table \ref{tab:spl_hotels} shows that test accuracy drops for 8 languages compared to \experimentIII except for Turkish, Chinese, and Japanese; whereas including gold English in \experimentII was helping most of the languages. This shows that our translated datasets are robust and informative enough that mixing them with data from another language would not improve the performance by a lot and in some cases can even hurt the results. The drop in the accuracy is caused due to two main reasons:\\
1) Our training dataset for each foreign language is generated by machine translation. The outputs are more natural-looking than synthesized English data even though they might not have correct grammar structure. Mixing distributions in train set is not a good approach especially since we validate and test on natural utterances.\\
2) The parameter values used in the foreign language are localized using our approach and are no longer in English. Thus seeing English examples with English parameters causes nothing but more confusion for the neural model's copying mechanism as we observe some English parameters present in the logical forms predicted by the model for the top 8 languages in Table~\ref{tab:spl_hotels}.

% since gold English sentences can be used to infer the correct program parameters and mitigates the structure and semantic noise introduced by direct translation. 
% \TODO{Discuss the numbers}

\subsection{Training with Human Translated Sentences}
As evident in Table~\ref{tab:bleu_hotels}, human translated data distribution is quite different from machine translated data. Can this difference be minimized by including human translated data in the training dataset in a few shot setting? Our hypothesis is that adding a few human utterances examples help the model generalizes better and avoids overfitting on uncommon sentence structures introduced by translation. 
 
\textbf{\experimentVII} In our final experiment, we concatenate the validation set obtained by humans to the training set generated using SPI. Since the validation size is much smaller than the training size (0.03\% for hotels and 0.12\% for restaurants) this is similar to a few-shot scenario where a small set of examples from eval/ test distribution are used for training.
We also create a new validation set by concatenating the machine and human translated examples from the validation set. This is to avoid overfitting on human data as we have included that in the training set. We then train the semantic parser on the joint train set and evaluate on the mixed development set. We experimented by evaluating only on machine translated validation data too but the results were lower. 

As shown in Table~\ref{tab:spl_hotels}, the test results are improved significantly across 9 languages for hotels domain achieving new state-of-the-art results on this benchmark. The improvement is partly due to low overlap between the train and test distributions as is evident by the low BLEU scores in Table\ref{tab:bleu_hotels} and partly due to few-shot and transfer capabilities of transformer models~\cite{brown2020language,campagna2020zeroshot,moradshahi2019hubert} attained via heavy pretraining on large corpora from different domains. 

We believe the parsing accuracy can be further boosted by adding more natural sentences collected via native speakers. We posit there is a threshold after which the cost of acquiring new examples outweighs the accuracy gain, but this investigation is out of the scope of this paper and will be explored in future work.

To summarize, in this section, we proposed several hypotheses and tested each by evaluating our methodology and comparing the results to other baseline methods.
\experimentI method proposed in \cite{bootstrap} performs poorly on 6 diverse languages. However, the results can be improved by including the original synthesized English data in the training since that mitigates the structure and semantic noise introduced by machine translation. We additionally perform a back translation of foreign languages test data into English and test the English semantic parser on them. The results outperform both baselines again for all 6 languages. Applying SPL achieves new best results for all the languages across all different settings. We observed choosing the best model evaluated on machine translated can yield similar human test performance compared to a model evaluated on human translated data for almost all languages. Adding gold English data did not help the \experimentIII results for almost all languages in contrast to the improvements obtained for \experimentII, speaking to the benefits of having training data instead of synthesized data for training. In fact, SPL translation method merges the two separate pipelines introduced in \cite{xu2020schema2qa} to generate the English dataset which is data synthesis and human paraphrasing. 
    
% \TODO{Discuss the numbers like the above.  What are the conclusions?}
 
%%%%%%%%%%
%%%% begin hotels
%%%%%%%%%%

